Model adaptation in a discrete fracture network: existence of solutions and numerical strategies

Fractures are normally present in the underground and are, for some physical processes, of paramount importance. Their accurate description is fundamental to obtain reliable numerical outcomes useful, e.g., for energy management. Depending on the physical and geometrical properties of the fractures, fluid flow can behave differently, going from a slow Darcian regime to more complicated Brinkman or even Forchheimer regimes for high velocity. The main problem is to determine where in the fractures one regime is more adequate than others. In order to determine these low-speed and high-speed regions, this work proposes an adaptive strategy which is based on selecting the appropriate constitutive law linking velocity and pressure according to a threshold criterion on the magnitude of the fluid velocity itself. Both theoretical and numerical aspects are considered and investigated, showing the potentiality of the proposed approach. From the analytical viewpoint, we show existence of weak solutions to such model under reasonable hypotheses on the constitutive laws. To this end, we use a variational approach identifying solutions with minimizers of an underlying energy functional. From the numerical viewpoint, we propose a one-dimensional algorithm which tracks the interface between the low- and high-speed regions. By running numerical experiments using this algorithm, we illustrate some interesting behaviors of our adaptive model on a single fracture and small networks of intersecting fractures.

==> interface1.tex <==
\section{Proposed model}\label{sec:proposed-model}

We identify our fracture network with an open, bounded connected set $\Omega \subset \R^d$ with Lipschitz boundary filled with a fluid of constant density $\rho \equiv 1$. Thus, mass conservation in $\Omega$ reads
\begin{equation}
  \label{eq:div-q}
  \dive \bu = q,
\end{equation}
where $\bu\: \Omega \to \R^d$ is the unknown velocity of the fluid and $q\: \Omega \to \R$ a given source term allowing, for instance, for fluid mass to be exchanged between the fractures and the surrounding porous medium. Note that we shall denote maps on $\Omega$ and their traces on the boundary $\p\Omega$ by the same notation. To \eqref{eq:div-q} we add the Neumann boundary condition
\begin{equation}
  \label{eq:neumann-cond}
  \bu \cdot \bn = b \quad \text{on $\p\Omega$},
\end{equation}
where $\bn$ is the outward normal unit vector of $\p\Omega$ and $b\:\p\Omega\to\R$ a given function.

\subsection{Velocity-pressure law}
\label{sec:vel-press-law}

Typically, one couples \eqref{eq:div-q} and \eqref{eq:neumann-cond} with a relation, or law, between the velocity field $\bu$ and the pressure field $p\: \Omega \to \R$ via some operator $\bLambda$:
\begin{equation}
  \label{eq:relation-u-p}
  \bLambda(\bu) = -\bgrad p + \bff,
\end{equation}
where $\bff$ is a given body force (e.g., gravity). Examples of laws $\bLambda$ relating velocity and pressure via \eqref{eq:relation-u-p} are
\begin{equation}\label{eq:F-ex}
  \begin{gathered}
    \bLambda_\mt{S}(\bu) = -\bLap \bu, \quad \bLambda_\mt{D}(\bu) = \bK^{-1} \bu,\\
    \quad \bLambda_\mt{B}(\bu) = -\bLap \bu + \bK^{-1} \bu, \quad \bLambda_\mt{DF}(\bu) = \bK^{-1} \bu + \alpha\abs{\bu}^{r-2}\bu,
  \end{gathered}
\end{equation}
where $\bK \: \Omega \to \R^{d\times d}$ is the permeability tensor and $\alpha\geq 0$ and $r\in\R_{\geq 2}$ some parameters. Choosing $\bLambda_\mt{S}$ gives Stokes' equation, $\bLambda_\mt{D}$ gives Darcy's equation, $\bLambda_\mt{B}$ gives Brinkman's equation and $\bLambda_\mt{DF}$ gives the generalized Darcy--Forchheimer equation (which simplifies into the common Darcy--Forchheimer when $r=3$).

The study of \eqref{eq:div-q} and \eqref{eq:neumann-cond} together with a law of the form \eqref{eq:relation-u-p} is very well-documented in the literature. \comment{referenze...} To the authors' knowledge, a known issue that has not yet found a documented answer is the case when one needs to choose a combination of laws such as those given as examples in \eqref{eq:F-ex}, rather than a single one, i.e., when one needs to couple different velocity-pressure laws according to some validity criterion which selects the better-adapted law. This criterion should depend on the speed regime (or Reynolds number) of the flow. For example, where the Reynolds number is low Darcy's law $\bLambda_\mt{D}$ may be preferred, whereas where it is high Stokes' equation $\bLambda_\mt{S}$ might be chosen instead. For this reason, in this paper we consider the case where we need to choose from two laws $\bLambda_1$ and $\bLambda_2$ according to some threshold speed $\bar u > 0$, which without loss of generality we take to be equal to $1$.

We write
\begin{equation}
  \begin{gathered}
    \Omega_1(\bu) = \{ \bx\in \Omega \st \abs{\bu(\bx)} < 1 \}, \quad \Omega_2(\bu) = \{ \bx\in \Omega \st \abs{\bu(\bx)} > 1\},\\ \Gamma(\bu) = \Omega\setminus (\Omega_1(\bu) \cup \Omega_2(\bu)) = \{\bx\in \Omega \st \abs{\bu(\bx)} = 1 \},
  \end{gathered}
\end{equation}
where $\Gamma(\bu)$ is referred  to as the \emph{interface}. Obviously, the family $\{\Omega_1(\bu),\Omega_2(\bu),\Gamma(\bu)\}$ forms a partition of $\Omega$. Because the velocity field is an unknown of the problem, the subdomains $\Omega_1(\bu)$ and $\Omega_2(\bu)$ and the interface $\Gamma(\bu)$ are also unknowns, directly depending on the velocity. We can rewrite these sets in a more compact form:
\begin{equation*}
  \Omega_1(\bu) = \bu^{-1}(B_1(\bnull)), \quad \Omega_1(\bu) = \bu^{-1}(\R^d\setminus B_1(\bnull)), \quad \Gamma(\bu) = \bu^{-1}(S_1(\bnull)),
\end{equation*}
where $B_1(\bnull)$ and $S_1(\bnull)$ stand respectively for the unit open ball and unit sphere in $\R^d$ centered at the origin $\bnull$. Note that if $\bu$ is not continuous, then $\Omega_1(\bu)$ and $\Omega_2(\bu)$ may not be open. Also note that, without further assumptions, the interface could be of any Hausdorff dimension less than or equal to $d$.

In this setting we can write our law operator $\bLambda$ in \eqref{eq:relation-u-p} as a combination of the operators $\bLambda_1$ and $\bLambda_2$ and an additional interface law operator $\bLambda_\Gamma$, such as
\begin{equation*}
  \bLambda(\bu) = \bLambda_1(\bu) \chi_{\Omega_1(\bu)} + \bLambda_2(\bu) \chi_{\Omega_2(\bu)} + \bLambda_\Gamma(\bu) \chi_{\Gamma(\bu)},
\end{equation*}
where $\chi_A$ is the indicator function of any set $A\subset\R^d$. The choice of the interface law seems to be aribitrary at this point, especially if we expect the interface to be of dimension lower than $d$. We might then be tempted to choose the zero law
\begin{equation*}
  \bLambda_\Gamma(\bu) = \bnull,
\end{equation*}
that is, to impose that the pressure has to satisfy $\bgrad p = \bff$ (and the velocity, by definition, $\abs{\bu} = 1$) on the interface. Another attempt, probably more satisfactory, would be to choose the interface law operator as a convex combination between $\bLambda_1$ and $\bLambda_2$, as in
\begin{equation}
  \label{eq:law-convex}
  \bLambda_\Gamma(\bu) = (1 - \tau) \bLambda_1(\bu) + \tau\bLambda_2(\bu),
\end{equation}
for some given $\tau\in[0,1]$, so that, for example, choosing $\tau=\tfrac12$ would mean that the interface law is the arithmetic average of the two ``main'' laws, yielding $\frac12 (\bLambda_1(\bu) + \bLambda_2(\bu)) + \bgrad p = \bff$ on the interface. A natural choice for $\bLambda_\Gamma$ stems from the following formal energetic consideration.

% In this convex combination setting, the law would take the form
% \begin{equation*}
%   \bLambda(\bu) = (1 - H_\tau(\abs{\bu})) \bLambda_1(\bu) + H_\tau(\abs{\bu}) \bLambda_2(\bu),
% \end{equation*}
% where $H_\tau\: \R \to \R$ is the Heaviside-like function defined for all $a\in\R$ by
% \begin{equation}
% \label{eq:heaviside-param}
%   H_\tau(a) =
%   \begin{cases}
%     0 & \text{if $a < 1$},\\
%     \tau & \text{if $a = 1$},\\
%     1 & \text{if $a > 1$}.
%   \end{cases}
% \end{equation}
% Taking a convex combination of the two ``main'' laws as in \eqref{eq:law-convex} within the interface seems to be a plausible choice as it ensures that the interface law operator is somewhat controlled by $\bLambda_1$ and $\bLambda_2$. When $d=1$, in fact, this combination makes sure that $\Lambda_\Gamma$ stays between $\Lambda_1$ and $\Lambda_2$. The issue with \eqref{eq:law-convex} is to decide where on the segment $[0,1]$ we should choose the parameter $\tau$, that is, which law along the convex combination between $\bLambda_1$ and $\bLambda_2$ we should choose. We may actually need to consider a function $\tau\: \Omega \to [0,1]$ as parameter rather than a fixed number; this is in fact the natural setting that emerges from a formal energetic consideration, as we explain below.

%  We cannot answer this point if we do not wish to give ourselves additional apriori knowledge on the interface. In this paper we will circumvent this issue by choosing a multivalued version of \eqref{eq:law-convex}, as described in Section \ref{sec:multiv-setting}.

% \begin{rem}
%   A further possible generalization of \eqref{eq:law-convex} would be to choose the interface law operator as a generic interpolation between $\bLambda_1$ and $\bLambda_2$ parametrized by some $h\in[0,1]$, as in
%   \begin{equation*}
%     \bLambda_\Gamma(\bu) = \bs{I}_h(\bLambda_1(\bu),\bLambda_2(\bu)),
%   \end{equation*}
%   where $(\bs{I}_h)_{h\in[0,1]}$ is a parametrized interpolator satisfying $\bs{I}_0(\ba,\bb) = \ba$ and $\bs{I}_1(\ba,\bb) = \bb$ for all $\ba,\bb\in\R^d$. Choosing $\bs{I}_h(\ba,\bb) = (1 - h) \ba + h\bb$ would recover the convex combination case \eqref{eq:law-convex}, whereas choosing
%   \begin{equation*}
%     \bs{I}_h(\ba,\bb) =  \abs{\ba}^h\abs{\bb}^{1-h} \left( \frac{(1-h)\ba}{\abs{\ba}} + \frac{h\bb}{\abs{\bb}} \right) \quad \text{or} \quad \bs{I}_h(\ba,\bb) = \left( \frac{1-h}{\abs{\ba}} + \frac{h}{\abs{\bb}} \right)^{-1} \left( \frac{(1-h)\ba}{\abs{\ba}} + \frac{h\bb}{\abs{\bb}} \right)
%   \end{equation*}
%   would give geometric-like or harmonic-like average laws, respectively. We choose not to explore this interpolated interface law in the present paper as it adds significant technical challenges to the convex combination case and we do not wish to study the interface in such depth at this point. We shall leave this issue, together with that of determining the dimensionality of the interface, for a subsequent paper.
% \end{rem}

\subsection{Formal energetic consideration}
\label{sec:energetic-cons}

Suppose that the law operators $\bLambda_1$ and $\bLambda_2$ take the forms
\begin{equation*}
  \bLambda_1(\bu) = \phi_1(\abs{\bu}^2)\bu \quad \text{and} \quad \bLambda_2(\bu) = \phi_2(\abs{\bu}^2)\bu,
\end{equation*}
where $\phi_1$ and $\phi_2$ are functions with enough regularity for the following consideration to hold. The classical setting is recovered here by taking $\phi_1 \equiv \phi_2 =: \phi$ and consequently $\bLambda_1 = \bLambda_2$. In this case it is known \comment{(referenza Spena-Vacca)} that, when $\phi$ is continuous and nondecreasing, solving \eqref{eq:div-q}--\eqref{eq:relation-u-p} is equivalent to minimizing on an adequate function space the energy
\begin{equation*}
  \E(\bu) = \int_\Omega \left( \Phi(\abs{\bu}^2) - \bff \cdot \bu \right),
\end{equation*}
where $\Phi$ is any primitive of $\tfrac\phi2$. Indeed, we have that $\E$ is differentiable and convex with gradient $\bgrad \E$ given by
\begin{equation*}
  \bgrad \E(\bu) = \phi(\abs{\bu}^2) \bu - \bff = \bLambda(\bu) - \bff,
\end{equation*}
so that minimizing $\E$ is equivalent to finding $\bu$ with $\bLambda(\bu) = \bff$, since in this case $\bgrad \E(\bu) =\bnull$. Writing
\begin{equation*}
  \D(\bu) = \int_\Omega \Phi(\abs{\bu}^2)
\end{equation*}
what is typically referred to as the dissipation functional, we see that $\bLambda(\bu) = \grad \D(\bu)$.

Following this approach in the general case where we may have $\phi_1 \not\equiv \phi_2$, the corresponding energy and dissipation are
\begin{equation*}
  \E(\bu) = \D(\bu) - \int_\Omega \bff\cdot\bu \quad \text{and} \quad \D(\bu) = \int_\Omega \left( \Phi_1(\abs{\bu}^2)\chi_{\Omega_1(\bu)} + \Phi_2(\abs{\bu}^2)\chi_{\Omega_2(\bu)} \right),
\end{equation*}
where and $\Phi_1$ and $\Phi_2$ are primitives of $\tfrac{\phi_1}{2}$ and $\tfrac{\phi_2}{2}$ to be chosen appropriately. Setting $\Psi(a) = \Phi_1(a)\chi_{a<1} + \Phi_2(a)\chi_{a>1}$ we can rewrite
\begin{equation*}
  \E(\bu) = \int_\Omega \left( \Psi(\abs{\bu}^2) - \bff\cdot\bu \right) \quad \text{and} \quad \D(\bu) = \int_\Omega \Psi(\abs{\bu}^2).
\end{equation*}
We note that $\Psi$ is continuous only provided that $\Phi_1(1) = \Phi_2(1) = 0$. We therefore choose the primitives $\Phi_1$ and $\Phi_2$ to be such that $\Phi_1(1) = \Phi_2(1) = 0$. When $\phi_1$ and $\phi_2$ are continuous and nondecreasing we notice that the Fréchet subdifferential $\p\E$ satisfies
\begin{equation*}
  \bp\E(\bu) = \begin{cases} \{\phi_1(\abs{\bu}^2)\bu - \bff\} = \{\bLambda_1(\bu) - \bff\}& \text{on $\Omega_1(\bu)$},\\ \{\phi_2(\abs{\bu}^2)\bu - \bff\} = \{\bLambda_2(\bu) - \bff\} & \text{on $\Omega_2(\bu)$}. \end{cases}
\end{equation*}
From subdifferential calculus we know that, even when $\E$ is not convex, a function $\bu$ is a local minimizer of $\E$ if and only if $\bnull \in \bp\E(\bu)$. This consideration therefore invites us to consider a multivalued setting where the law operator $\bLambda$ is in fact the \emph{set} of operators given by the subdifferential of $\D$:
\begin{equation*}
  \bLambda(\bu) = \bp\D(\bu).
\end{equation*}
This is the setting we choose for the rest of the paper.
% In this case, we also note that when $\phi_1$ and $\phi_2$ are convex and $\phi_1(1) \leq \phi_2(1)$ the energy $\E$ is convex and its subdifferential $\p\E$ is given, as we will prove later, by
% \begin{align*}
%   \p \E(\bu) &= (1 - \frakH(\abs{\bu}^2)) \phi_1(\abs{\bu}^2) \bu + \frakH(\abs{\bu}^2) \phi_2(\abs{\bu}^2) \bu - \bff\\
%   &= (1 - \frakH(\abs{\bu}^2)) \bLambda_1(\bu) + \frakH(\abs{\bu}^2) \bLambda_2(\bu) - \bff,
% \end{align*}
% where $\frakH \: \R \to 2^{L^\infty(\Omega;[0,1])}$ is defined for all $a\in\R$ as
% \begin{equation}
%   \label{eq:heaviside-multiv}
%   \frakH(a) =
%   \begin{cases}
%     \{0\} & \text{if $a < 1$},\\
%     L^\infty(\Omega;[0,1]) & \text{if $a = 1$},\\
%     \{1\} & \text{if $a > 1$}.
%   \end{cases}
% \end{equation}
% (Within the above curly brackets, $0$ and $1$ stand respectively for the zero and one constant functions, which of course belong to $L^\infty(\Omega;[0,1])$.)


\section{Mathematical setting}
\label{sec:math-setting}

We give in this section the rigorous mathematical setting we consider, in particular we introduce the assumptions on the underlying law operator as well as the weak formulation of our problem.

\subsection{Assumptions and strong formulation}
\label{sec:assu-vel-press}

Let $\phi_1,\phi_2\: [0,\infty) \to [0,\infty)$ be continuous, convex and strictly increasing on $[0,1]$ and $[1,\infty)$, respectively. Furthermore, suppose that $\phi_2$ satisfies the following assumption: there exist $r\geq 2$ and $c,C>0$ such that
\begin{equation}
  \label{eq:bound-phi2}
   c a^{\frac{r-2}{2}} \leq \phi_2(a) \leq C \left(1+a^{\frac{r-2}{2}}\right) \quad \text{for all $a\geq 1$}.
\end{equation}
We write $\Psi\:[0,\infty)\to \R$ the function given by
\begin{equation*}
  \Psi(a) = \begin{cases} \Phi_1(a) & \text{for all $a< 1$},\\ 0 & \text{for $a=1$},\\ \Phi_2(a) & \text{for all $a> 1$}, \end{cases}
\end{equation*}
where $\Phi_1,\Phi_2\:[0,\infty) \to \R$ are primitives of $\tfrac{\phi_1}{2}$ and $\tfrac{\phi_2}{2}$ such that $\Phi_1(1) = \Phi_2(1) = 0$. We define the dissipation $\D\:\bL^r(\Omega) \to \R$ by
\begin{equation}
  \label{eq:dissipation}
  \D(\bu) = \int_\Omega \Psi(\abs{\bu}^2) \quad \text{for all $\bu\in \bL^r(\Omega)$}.
\end{equation}
\comment{[Mostrare che in effetti $\dom\D = \bL^r(\Omega)$.]}
% In the following, the operator laws $\bLambda_1$ and $\bLambda_2$ are assumed to be of the form
% \begin{equation}
% \label{eq:law-form}
%   \bLambda_1(\bu) = \phi_1(\abs{\bu}^2)\bu \quad \text{and} \quad \bLambda_2(\bu) = \phi_2(\abs{\bu}^2) \bu,
% \end{equation}
% where
% Our combined law $\bLambda$ defined in \eqref{eq:multiv-heaviside-law} maps $\bL^r(\Omega)$ to the power set $2^{\bL^s(\Omega)}$. Indeed, let $\bu\in\bL^r(\Omega)$ and $\bLambda_{\bu} \in \bLambda(\bu)$ and write $\tau\in L^\infty(\Omega;[0,1])$ such that $\bLambda_{\bu} = \bLambda(\tau;\bu)$; then, writing $\sigma = \sup_{a\in[0,1]}\phi_1(a)$, which is finite thanks to the continuity of $\phi_1$, and using the right-hand inequality in \eqref{eq:bound-phi2} and the fact that $1 < s \leq r$, we get
% \begin{align*}
%   \norm{\bLambda_{\bu}}_{\bL^s(\Omega)}^s &= \int_{\Omega_1(\bu)} \abs{\phi_1(\abs{\bu}^2)\bu}^s + \int_{\Omega_2(\bu)} \abs{\phi_2(\abs{\bu}^2)\bu}^s + \int_{\Gamma(\bu)} \abs{((1-\tau) \lambda_1 + \tau\lambda_2)\bu}^s\\
%   &\leq \sigma^s \int_{\Omega_1(\bu)} \abs{\bu}^s + 2^{s-1}C^s\int_{\Omega_2(\bu)} \abs{\bu}^s + 2^{s-1}C^s\int_{\Omega_2(\bu)} \abs{\bu}^r  + \max\{\lambda_1,\lambda_2\}^s \int_{\Gamma(\bu)}\abs{\bu}^s\\
%   &\leq \sigma^s \abs{\Omega} + 2^{s-1}C^s\int_{\Omega_2(\bu)} \abs{\bu}^r + 2^{s-1}C^s\int_{\Omega_2(\bu)} \abs{\bu}^r  + \max\{\lambda_1,\lambda_2\}^s \abs{\Omega}\\
%   &\leq 2^sC^s\norm{\bu}_{\bL^r(\Omega)}^r + (\sigma^s + \max\{\lambda_1,\lambda_2\}^s)\abs{\Omega} <\infty.
% \end{align*}
We write $\bLambda = \bp\D$, where $\bp\D$ is the Fréchet subdifferential of $\D$; we refer to $\bLambda$ as the velocity-pressure law operator. \comment{[Dare la definizione di sottodifferenziale.]} Indeed, our problem is the following: find a pair $(\bu,p)\in \bL^r(\Omega)\times W^{1,s}(\Omega)$ such that
\begin{equation}
  \label{eq:main}
  \begin{gathered}
    \dive \bu = q \quad \text{on $\Omega$},\\
    -\bgrad p + \bff \in \bLambda(\bu) \quad \text{on $\Omega$},\\
    \bu \cdot \bn = b \quad \text{on $\p\Omega$},
  \end{gathered}
\end{equation}
where $s = \tfrac{r}{r-1}$ is the conjugate exponent of $r$. In view of \eqref{eq:main}, we impose
\begin{equation*}
  \bff\in \bL^s(\Omega), \quad q \in L^r(\Omega) \quad \text{and} \quad b \in L^r(\p\Omega),
\end{equation*}

\begin{rem}
  This setting physically restricts us to scalar permabilities. Indeed, the underlying law operators $\bLambda_1$ and $\bLambda_2$ of Section \ref{sec:proposed-model} are here of the form
\begin{equation*}
  \bLambda_1(\bu) = \phi_1(\abs{\bu}^2)\bu \quad \text{and} \quad \bLambda_2(\bu) = \phi_2(\abs{\bu}^2)\bu,
\end{equation*}
as discussed in \ref{sec:energetic-cons}. More general laws including tensor permeabilities, as motivated in \comment{Spena-Vacca}, are for instance given by the following:
  \begin{equation*}
    \bLambda_1(\bu) = \phi_1(\blambda_1\bu\cdot\bu)\blambda_1\bu,
  \end{equation*}
and analogously for $\bLambda_2$, where $\blambda_1\in\R^{d\times d}$ is a symmetric positive definite matrix encoding a tensor permeability. Even more general forms are envisageable:
\begin{equation*}
    \bLambda_1(\bu) = \sum_{j=1}^n \phi_{1,j}(\blambda_{1,j}\bu\cdot\bu)\blambda_{1,j}\bu,
  \end{equation*}
where the $\phi_{1,j}$ and $\blambda_{1,j}$ are $n$ different law functions and permeability tensors. We leave these general laws to a future work. We claim that the techniques we use in the present paper for scalar laws should extend to tensor laws without too much difficulty.
\end{rem}

In the rest of the paper we shall write
\begin{equation}
  \label{eq:lambdas}
  \lambda_1 := \phi_1(1) \quad \text{and} \quad \lambda_2 := \phi_2(1).
\end{equation}


\subsection{Weak formulation}
\label{sec:weak-formulation}

Problem \eqref{eq:main} in its weak formulation is the following: find $(\bu,p)\in \bL^r(\Omega)\times W^{1,s}(\Omega)$ so that there exists $\bLambda_{\bu} \in \bLambda(\bu)$ such that for all $\bvarphi\in \bL^r(\Omega)$ and $\psi\in W^{1,s}(\Omega)$ there holds
\begin{equation}
  \label{eq:weak-form}
  \begin{gathered}
    \int_\Omega \bLambda_{\bu} \cdot \bvarphi = - \int_\Omega \bgrad p \cdot\bvarphi + \int_\Omega \bff\cdot\bvarphi,\\
    \int_\Omega \bgrad \psi\cdot \bu = -\int_\Omega q\psi + \int_{\p\Omega} b\psi.
  \end{gathered}
\end{equation}
We shall equivalently manipulate functions in $\bL^s(\Omega)$ as elements of $(\bL^r(\Omega))^*$, the dual of $\bL^r(\Omega)$. In particular, this means that, given $\bu\in \bL^r(\Omega)$, operators $\bLambda_{\bu}$ in $\bLambda(\bu)$ will also be seen as maps from $\bL^r(\Omega)$ to $(\bL^r(\Omega))^* \sim \bL^s(\Omega)$. Writing $\ap{\cdot,\cdot}$ the dual mapping on $\bL^s(\Omega)\times \bL^r(\Omega)$, the weak formulation in \eqref{eq:weak-form} of our problem can be restated as follows: find $(\bu,p)\in \bL^r(\Omega)\times W^{1,s}(\Omega)$ so that there exists $\bLambda_{\bu} \in \bLambda(\bu)$ such that for all $\bvarphi\in \bL^r(\Omega)$ and $\psi\in W^{1,s}(\Omega)$ there holds
\begin{equation}
  \label{eq:weak-form-main}
  \begin{gathered}
    \ap{\bLambda_{\bu},\bvarphi} = -\ap{\bgrad p,\bvarphi} + \ap{\bff,\bvarphi},\\
    \ap{\bgrad\psi,\bu} = - \int_\Omega q\psi + \int_{\p\Omega} b\psi .
  \end{gathered}
\end{equation}
Our goal is now to show well-posedness for this weak formulation.


% \subsection{Multivalued setting}
% \label{sec:multiv-setting}

% As argued previously, the law operator $\bLambda$ is from this point allowed to be multivalued, so that the velocity-pressure law in \eqref{eq:relation-u-p} actually reads
% \begin{equation}
%   \label{eq:multiv-law}
%   -\bgrad p + f \in \bLambda(\bu).
% \end{equation}
% We are thus allowed to take the following set of convex combinations between $\bLambda_1$ and $\bLambda_2$ as our interface law operator, as suggested by the energetic consideration of Section \ref{sec:energetic-cons}:
% \begin{equation*}
%   \bLambda_\Gamma(\bu) = \left\{ (1 - \tau) \bLambda_1(\bu) + \tau\bLambda_2(\bu) \right\}_{\tau\in L^\infty(\Omega;[0,1])}.
% \end{equation*}
% In other terms, our law operator $\bLambda$ satisfies
% \begin{equation}
%   \label{eq:multiv-heaviside-law}
%   \bLambda(\bu) = (1 - \frakH(\abs{\bu}^2)) \bLambda_1(\bu) + \frakH(\abs{\bu}^2) \bLambda_2(\bu) = \bLambda_1(\bu) + \frakH(\abs{\bu}^2) (\bLambda_2(\bu) - \bLambda_1(\bu)),
% \end{equation}
% where $\frakH \: \R \to 2^{L^\infty(\Omega;[0,1])}$ is given in \eqref{eq:heaviside-multiv}. Our problem thus summarizes as: find a pair $(\bu,p)$ of functions such that
% \begin{equation}
%   \label{eq:main}
%   \begin{gathered}
%     \dive \bu = q \quad \text{on $\Omega$},\\
%     -\bgrad p + \bff \in \bLambda(\bu) \quad \text{on $\Omega$},\\
%     \bu \cdot \bn = b \quad \text{on $\p\Omega$},
%   \end{gathered}
% \end{equation}
% where the law operator $\bLambda$ is of the form \eqref{eq:multiv-heaviside-law}. For any $\tau\in L^\infty(\Omega;[0,1])$ we shall denote by $\frakH_\tau\:\R\to L^\infty(\Omega;[0,1])$ the function defined for all $a\in\R$ by
% \begin{equation*}
%   \frakH_\tau(a) =
%   \begin{cases}
%     0 & \text{if $a < 1$},\\
%     \tau & \text{if $a = 1$},\\
%     1 & \text{if $a > 1$},
%   \end{cases}
% \end{equation*}
% and
% \begin{equation*}
%   \bLambda(\tau;\bu) = (1 - \frakH_\tau(\abs{\bu}^2)) \bLambda_1(\bu) + \frakH_\tau(\abs{\bu}^2) \bLambda_2(\bu) = \bLambda_1(\bu) + \frakH_\tau(\abs{\bu}^2) (\bLambda_2(\bu) - \bLambda_1(\bu)).
% \end{equation*}
% With this, our problem amounts to: find a triplet $(\bu,p,\tau)$ with $\tau\in L^\infty(\Omega;[0,1])$ such that
% \begin{equation}
%   \label{eq:main-tau}
%   \begin{gathered}
%     \dive \bu = q \quad \text{on $\Omega$},\\
%     -\bgrad p + \bff = \bLambda(\tau;\bu) \quad \text{on $\Omega$},\\
%     \bu \cdot \bn = b \quad \text{on $\p\Omega$}.
%   \end{gathered}
% \end{equation}


\section{Well-posedness}
\label{sec:well-posedness}

Let us introduce the set $\bV_0$ given by
\begin{equation*}
  \bV_0 = \{ \bvarphi \in \bL^r(\Omega) \st \forall\, \psi\in W^{1,s}(\Omega),\, \ap{\bgrad \psi,\bvarphi} = 0 \}.
\end{equation*}
We also define the maps $B \in \bL^r(\Omega) \to (W^{1,s}(\Omega))^*$ and $\bB^* \: W^{1,s}(\Omega) \to (\bL^r(\Omega))^*$  by
\begin{equation}
  \label{eq:B}
  B(\bvarphi)(\psi) = \bB^*(\psi)(\bvarphi) = \ap{\bgrad \psi, \bvarphi} \quad \text{for all $\bvarphi \in \bL^r(\Omega)$ and $\psi\in W^{1,s}(\Omega)$},
\end{equation}
In particular, we have $\bV_0 = \mathrm{Ker}(B)$.

\subsection{Preliminaries}
\label{sec:preliminaries-well-posedness}

Via the following two lemmas, we simplify our weak formulation \eqref{eq:weak-form-main} into a problem restricted to $\bV_0$ (cf. \eqref{eq:weak-form-V0} below).
\begin{lem}
  \label{lem:bdry-V0}
  There exists a unique $\bu_\perp\in \bV_0^{\mt{\perp}}$ such that
  \begin{equation*}
    \ap{\bgrad \psi,\bu_\perp} = -\int_\Omega q\psi + \int_{\p\Omega} b\psi \quad \text{for all $\psi\in W^{1,s}(\Omega)$}.
  \end{equation*}
\end{lem}
\begin{proof}
  \comment{da scrivere, seguire la proposizione 3.1 in AFM.}
\end{proof}
\begin{lem}
  The weak formulation \eqref{eq:weak-form-main} is equivalent to the following problem: find $\bv\in \bV_0$ such that there exists $\bLambda_{\bu} \in \bLambda(\bv+\bu_\perp)$ satisfying
  \begin{equation}
    \label{eq:weak-form-V0}
    \ap{\bLambda_{\bu},\bvarphi} = \ap{\bff,\bvarphi} \quad \text{for all $\bvarphi \in \bV_0$},
  \end{equation}
  where $\bu_\perp$ is given by Lemma \ref{lem:bdry-V0}.
\end{lem}
\begin{proof}
  We first suppose that $(\bu,p)$ is solution to Problem \eqref{eq:weak-form-main}. Then we decompose $\bu$ as $\bu = (\bu - \bu_\perp) + \bu_\perp =: \bv + \bu_\perp$. By \eqref{eq:weak-form-main}, there exists $\bLambda_{\bu} \in \bLambda(\bu) = \bLambda(\bv+\bu_\perp)$ such that
  \begin{equation*}
    \ap{\bLambda_{\bu},\bvarphi} = \ap{\bff,\bvarphi} \quad \text{for all $\bvarphi \in \bV_0$}.
  \end{equation*}
Furthermore, for all $\psi\in W^{1,s}(\Omega)$ we find $\ap{\bgrad\psi,\bv} = \ap{\bgrad\psi,\bu} - \ap{\bgrad\psi,\bu_\perp} = 0$, so that $\bv\in \bV_0$ and $\bv$ satisfies Problem \eqref{eq:weak-form-V0}.

  Suppose now that $\bv$ satisfies Problem \eqref{eq:weak-form-V0}. Then, $\bLambda_{\bu} - \bff \in \bV_0^{\mathrm{\perp}}$. By the fact that $\bV_0 = \mathrm{Ker}(B)$, where $B$ is defined in \eqref{eq:B}, the closed-range theorem ensures that $\bV_0^{\mathrm{\perp}} = \mt{Im}(\bB^*)$, where $\bB^*$ is also defined in \eqref{eq:B}. Because $\bB^*$ is an isomorphism from $W^{1,s}(\Omega)$ to its image  \comment{[referenza]}, there exists a unique $p\in W^{1,s}(\Omega)$ such that
  \begin{equation*}
    \ap{\bLambda_{\bu} - \bff,\bvarphi} = \bB^*(-p)(\bvarphi) = -\ap{\bgrad p,\bvarphi} \quad \text{for all $\bvarphi\in\bL^r(\Omega)$}.
  \end{equation*}
Then, writing $\bu = \bv + \bu_\perp$ we get
\begin{equation*}
  \ap{\bgrad\psi,\bu} = \ap{\bgrad\psi,\bv} + \ap{\bgrad\psi,\bu_\perp} = \ap{\bgrad\psi,\bu_\perp}  = - \int_\Omega q\psi + \int_{\p\Omega} b\psi,
\end{equation*}
since $\bv\in \bV_0$. We thus have that $(\bu,p)$ satisfies Problem \eqref{eq:weak-form-main}, with $p$ unique.
\end{proof}

In the following we write $\bLambda_0\:\bV_0 \to (\bV_0)^*$ the operator given by
\begin{equation*}
  \bLambda_0(\bv) = \bLambda(\bv + \bu_\perp) \quad \text{for all $\bv\in\bV_0$},
\end{equation*}
where $\bu_\perp$ is defined as in Lemma \ref{lem:bdry-V0}. Similarly, we write $\D_0\:\bV_0 \to \R$ and $\E_0\:\bV_0 \to \R$ the functionals given by
\begin{equation*}
  \D_0(\bv) = \D(\bv + \bu_\perp) \quad \text{and} \quad \E_0(\bv) = \D_0(\bv) - \ap{\bff,\bv} \quad \text{for all $\bv\in\bV_0$}.
\end{equation*}
% Similarly, for $i\in\{1,2\}$,  we define $\bLambda_{0,i}\:\bV_0 \to (\bV_0)^*$ as
% \begin{equation*}
%   \bLambda_{0,i}(\bv) = \bLambda_i(\bv + \bu_\perp) \quad \text{for all $\bv\in\bV_0$},
% \end{equation*}


\subsection{Results}
\label{sec:results-well-posedness}

We state and prove here our results on existence and uniqueness for Problem \eqref{eq:weak-form-V0}, which thanks to Lemma \ref{lem:bdry-V0} are in fact existence and uniqueness results on Problem \eqref{eq:weak-form-main}. We will see that our results strongly depend on sign of the difference $\lambda_2 - \lambda_1$ (cf. \eqref{eq:lambdas}).

\subsubsection{Case $\lambda_1\leq\lambda_2$}
\label{sec:case-1-less-than-2}

The result we wish to show here is the following:
\begin{thm}[Existence and uniqueness when $\lambda_1 \leq \lambda_2$]
  \label{thm:wp-1-less-than-2}
  Suppose that $\lambda_1 \leq \lambda_2$. Then, Problem \eqref{eq:weak-form-V0} has a unique solution.
\end{thm}
Before giving the proof of this theorem, we recall that Problem \eqref{eq:weak-form-V0} has an equivalent formulation in terms of a minimization problem. Consider the following minimization problem: find $\bv\in\bV_0$ such that
\begin{equation}
  \label{eq:minimization}
  \E_0(\bv) = \inf_{\bw\in\bV_0} \E_0(\bw).
\end{equation}
\begin{lem}
  \label{lem:equivalence-min}
  Problems \eqref{eq:weak-form-V0} and \eqref{eq:minimization} are equivalent.
\end{lem}
\begin{proof}
  \comment{Diretto dalla definizione di sottodifferenziale. Da scrivere.}
\end{proof}

We can now prove Theorem \ref{thm:wp-1-less-than-2}.
\begin{proof}[Proof of Theorem \ref{thm:wp-1-less-than-2}]
  In this case, the integrand $\Psi$ in $\D_0$ is convex, so that $\D$ is \emph{strictly} convex. An application of the direct method of the calculus of variations yields the existence of a unique minimizer for Problem \ref{eq:minimization}. By Lemma \ref{lem:equivalence-min} we end the proof. \comment{[Dare tutti i dettagli]}
\end{proof}



\subsubsection{Case $\lambda_1 > \lambda_2$}
\label{sec:case-2-less-than-1}

This case is more difficult to tackle than the case $\lambda_1 \leq \lambda_2$. Indeed, we lose here the convexity of the integrand $\Psi$, which by Tonelli's theorem of functional analysis means that $\D_0$ is not weakly lower semicontinuous. As a consequence we cannot use the direct method of the calculus of variations to deduce the existence of a minimizer to $\E_0$.

\comment{Idea:

Our strategy is the following. We define a secondary minimization problem on the functional $\hat \E_0$ defined by
\begin{equation*}
  \hat \E_0(\bv) = \int_\Omega \hat\Psi(\abs{\bv+\bu_\perp}^2) - \ap{\bff,\bv},
\end{equation*}
where $\hat \Psi$ is the convex envelope of $\Psi$. (This should correspond to the double convex conjugate of $\Psi$.) Then $\hat\Psi \leq \Psi$ and $\hat \Psi$ is differentiable and convex. Because $\Psi$ is piecewise convex on the intervals $[0,1]$ and $[1,\infty)$ we actually have values $\hat \lambda_1 < 1$ and $\hat \lambda_2 > 1$ such that
\begin{equation*}
  \hat\Psi(a) = \Psi(a) \quad \text{for all $a<\hat\lambda_1$ and $a>\hat\lambda_2$}.
\end{equation*}
$\hat\E_0$ has a unique minimizer $\hat\bv$. We have the following result:
\begin{thm}[Existence and uniqueness when $\lambda_1 > \lambda_2$]
  Suppose that $\lambda_1 > \lambda_2$. Suppose that $\hat\bv$ satisfies the following condition:
  \begin{equation*}
    \abs{\hat \bv(x)} \not\in [\hat\lambda_1,\hat \lambda_2] \quad \text{for almost every $\bx\in\Omega$}.
  \end{equation*}
Then, Problem \eqref{eq:weak-form-V0} has a unique solution.
\end{thm}
\begin{proof}
  We have in this case, for all $\bv\in\bV_0$,
  \begin{equation*}
    \E_0(\hat\bv) = \hat\E_0(\hat\bv) \leq \hat \E_0(\bv) \leq \E_0(\bv).
  \end{equation*}
  Thus $\hat\bv$ is a minimizer of $\E_0$. Because a convex analysis theorem tells us that $\inf \hat\E_0 = \inf \E_0$, this must be the unique minimizer of $\E_0$ (check...).
\end{proof}

In the Darcy-Darcy case, this condition on $\hat \bv$ should hold when $\bff\in\bV_0^\perp$.
}


\comment{Questions for later (with student?):
  \begin{itemize}
    \item Which law in $\bp D$ is being picked at the interface?
    \item Extend the result to tensor permeabilities.
    \item Can we add $p$ in the law operator?
    \item What is the dimension of the interface?
  \end{itemize}
}

% The proof of this theorem will be based on the multivalued version of the Minty--Browder theorem \comment{referenza}, which we recall reads as follows:
% \begin{thm}[Minty--Browder]
%   Let $X$ be a reflexive Banach space with dual $X^*$. Let $T_1\: X \to X^*$ be a single-valued, bounded, coercive, hemicontinuous, monotone operator with $\dom(T_1) = X$. Let furthermore $T_2 \: X \to 2^{X^*}$ be a multivalued maximal monotone operator with $\dom(T_2) = X$. Then, the image of the multivalued operator $T_1 + T_2$ is all of $X^*$, i.e., for all $y\in X^*$ there exists $x\in X$ such that $y\in T(x)$.
% \end{thm}

% Note first that because $\bV_0$ is closed and $\bL^r(\Omega)$ is reflexive, $\bV_0$ is also reflexive. Recalling \eqref{eq:multiv-heaviside-law} we see that our law on $\bV_0$ can be written
% \begin{equation*}
%   \bLambda_0 = \bLambda_{0,1} + \bLambda_{0,21},
% \end{equation*}
% where $\bLambda_{0,21} \: \bV_0 \to (\bV_0)^*$ is the multivalued operator defined by
% \begin{equation*}
%   \bLambda_{0,21}(\bv) = \frakH(\abs{\bv + \bu_\perp}^2)(\bLambda_{0,2}(\bv) - \bLambda_{0,1}(\bv)) \quad \text{for all $\bv\in \bV_0$}.
% \end{equation*}
% The existence part of Theorem \ref{thm:wp-1-less-than-2} would be a direct consequence of $\bLambda_{0,1}$ being bounded, coercive, hemicontinuous and monotone on the one hand, and $\bLambda_{0,21}$ being maximal on the other hand. We focus on this task in the next two lemmas.

% \begin{lem}
%   The operator $\bLambda_{0,1}$ is bounded, coercive, hemicontinuous and monotone.
% \end{lem}
% \begin{proof}
%   We show in order that $\bLambda_{0,1}$ is bounded, coercive, hemicontinuous and monotone.

%   \medskip
%   \noindent \ul{Boundedness.} We want to show that $\bLambda_{0,1}$ maps bounded sets of $\bV_0$ to bounded sets of $(\bV_0)^*$. To this end, let $\bv\in\bV_0$ be such that $\norm{\bv}_{\bL^r(\Omega)} \leq R$ for some $R>0$. Thanks to \eqref{eq:bound-phi2} and \eqref{eq:bound-phi1}, setting $\bu = \bv + \bu_\perp$ and $\sigma = \sup_{a\in[0,1]}\phi_1(a)$ we get
%   \begin{align*}
%     \norm{\bLambda_{0,1}(\bv)}_{\bL^s(\Omega)}^s &= \norm{\phi_1(\abs{\bu}^2)\bu}_{\bL^s(\Omega)}^s = \int_\Omega \abs{\phi_1(\abs{\bu}^2)\bu}^s\\
%     &\leq \sigma^s \int_{\Omega_1(\bu)} \abs{\bu}^s + \int_{\Omega_2(\bu)} \abs{\phi_1(\abs{\bu}^2)\bu}^s + \int_{\Gamma(\bu)} \abs{\phi_1(\abs{\bu}^2)\bu}^s\\
%     &\leq \sigma^s \int_\Omega \abs{\bu}^s + \int_\Omega \abs{\phi_1(\abs{\bu}^2)\bu}^s + \lambda_1^s \abs{\Omega}\\
%     &\leq \sigma^s\norm{\bu}_{\bL^s(\Omega)}^s + 2^{1-s} C^s \left( \int_\Omega \abs{\bu}^{(r-1)s} + \int_\Omega \abs{\bu}^s \right) + \lambda_1^s \abs{\Omega}\\
%     &= \sigma^s\norm{\bu}_{\bL^s(\Omega)}^s + 2^{1-s} C^s\left( \norm{\bu}_{\bL^r(\Omega)}^r + \norm{\bu}_{\bL^s(\Omega)}^s \right) + \lambda_1^s \abs{\Omega}\\
%     &\leq C_\Omega \sigma^s\norm{\bu}_{\bL^r(\Omega)}^s + 2^{1-s} C^s (\norm{\bu}_{\bL^r(\Omega)}^r + C_\Omega \norm{\bu}_{\bL^r(\Omega)}^s) + \lambda_1^s \abs{\Omega}\\
%     &\leq 2^{1-s} C^s (\norm{\bv}_{\bL^r(\Omega)} + \norm{\bu_\perp}_{\bL^r(\Omega)})^r + C_\Omega(2^{1-s} C^s + \sigma^s) (\norm{\bv}_{\bL^r(\Omega)}+ \norm{\bu_\perp}_{\bL^r(\Omega)})^s + \lambda_1^s \abs{\Omega}\\
%     &\leq 2^{1-s} C^s (R + \norm{\bu_\perp}_{\bL^r(\Omega)})^r + C_\Omega(2^{1-s} C^s + \sigma^s) (R+ \norm{\bu_\perp}_{\bL^r(\Omega)})^s + \lambda_1^s \abs{\Omega},
%   \end{align*}
%   where $C_\Omega>0$ is a constant depending on the Lebesgue measure of the bounded set $\Omega$, so that
%   \begin{equation*}
%     \norm{\bLambda_{0,1}(\bv)}_{\bL^s(\Omega)} \leq (2^{1-s} C^s (R + \norm{\bu_\perp}_{\bL^r(\Omega)})^r + C_\Omega(2^{1-s} C^s + \sigma^s) (R+ \norm{\bu_\perp}_{\bL^r(\Omega)})^s + \lambda_1^s \abs{\Omega})^{1/s} < \infty.
%   \end{equation*}
%   By arbitrariness of $R$, this yields the boundedness of $\bLambda_{0,1}$.

%   \medskip
%   \noindent \ul{Coercivity.} Let $\bv\in\bV_0$. Then, again setting $\bu = \bv + \bu_\perp$ and $\sigma = \sup_{a\in[0,1]} \phi_1(a)$, we have
%   \begin{align*}
%     \ap{\bLambda_{0,1}(\bv),\bv} &= \int_\Omega \phi_1(\abs{\bu}^2) \bu\cdot \bv = \int_\Omega \phi_1(\abs{\bu}^2) \bu\cdot \bu - \int_\Omega \phi_1(\abs{\bu}^2) \bu \cdot \bu_\perp\\
%     &\geq \int_{\Omega_2(\bu)} \phi_1(\abs{\bu}^2) \abs{\bu}^2 - \int_\Omega \bLambda_{0,1}(\bv) \cdot \bu_\perp\\
%     &= \int_{\Omega} \phi_1(\abs{\bu}^2) \abs{\bu}^2 - \int_{\Omega_1(\bu)} \phi_1(\abs{\bu}^2) \abs{\bu}^2 - \int_{\Gamma(\bu)} \phi_1(\abs{\bu}^2) \abs{\bu}^2 - \int_\Omega \bLambda_{0,1}(\bv) \cdot \bu_\perp\\
%     &\geq \int_{\Omega} \phi_1(\abs{\bu}^2) \abs{\bu}^2 - (\sigma+\lambda_1) \abs{\Omega} - \norm{\bLambda_{0,1}(\bv)}_{\bL^s(\Omega)}\norm{\bu_\perp}_{\bL^r(\Omega)}\\
%     &\geq c\norm{\bu}_{\bL^r(\Omega)}^r - (\sigma+\lambda_1) \abs{\Omega} - \norm{\bLambda_{0,1}(\bv)}_{\bL^s(\Omega)}\norm{\bu_\perp}_{\bL^r(\Omega)}.
%   \end{align*}
%   Following the above computation for boundedness, we further get
%   \begin{align*}
%     \ap{\bLambda_{0,1}(\bv),\bv} &\geq c \norm{\bv+\bu_\perp}_{\bL^r(\Omega)}^r\\
%     &\quad - (2^{1-s} C^s (R + \norm{\bu_\perp}_{\bL^r(\Omega)})^r + C_\Omega(2^{1-s} C^s + \sigma^s) (R+ \norm{\bu_\perp}_{\bL^r(\Omega)})^s + \lambda_1^s \abs{\Omega})^{1/s}\norm{\bu_\perp}_{\bL^r(\Omega)}\\
%     &\geq c \norm{\bv+\bu_\perp}_{\bL^r(\Omega)}^r - P(\norm{\bv}_{\bL^r(\Omega)}),
%   \end{align*}
%   for some $P\:\R \to \R$ such that $P(a)a^{1-r} \to p$ as $a\to\infty$, with $p\in \R$, and so, when $\bv\neq\bnull$,
%    \begin{equation*}
%      \frac{\ap{\bLambda_{0,1}(\bv),\bv}}{\norm{\bv}_{\bL^r(\Omega)}} \geq c \frac{\norm{\bv+\bu_\perp}_{\bL^r(\Omega)}^r}{\norm{\bv}_{\bL^r(\Omega)}} - \frac{P(\norm{\bv}_{\bL^r(\Omega)})}{\norm{\bv}_{\bL^r(\Omega)}} = c \norm{\bv}_{\bL^r(\Omega)}^{r-1} + Q(\norm{\bv}_{\bL^r(\Omega)}),
%    \end{equation*}
%    for some $Q\:\R \to \R$ such that $Q(a)a^{2-r}\to q$ as $a\to\infty$, with $q\in\R$. We therefore get
%    \begin{equation*}
%      \frac{\ap{\bLambda_{0,1}(\bv),\bv}}{\norm{\bv}_{\bL^r(\Omega)}} \to \infty \quad \text{as $\norm{\bv}_{\bL^r(\Omega)} \to \infty$},
%    \end{equation*}
%    which shows coercivity of $\bLambda_{0,1}$.

%    \medskip
%    \noindent \ul{Hemicontinuity.} Let $\bv,\bw,\bvarphi\in\bV_0$. Define $L\:[0,1] \to \R$ and $\bL \: [0,1] \to \bL^s(\Omega)$ by
%    \begin{equation*}
%      L(t) = \ap{\bL(t),\bvarphi} = \ap{\bLambda_{0,1}(\bv+t\bw),\bvarphi} \quad \text{for all $t\in[0,1]$}.
%    \end{equation*}
%    Let $t\in[0,1]$ and write $\bu = \bv + \bu_\perp$. Then,
%    \begin{align*}
%      \abs{\bL(t)} &= \abs{\bLambda_{0,1}(\bv+t\bw)} = \abs{\phi_1(\abs{\bu + t\bw}^2)(\bu+t\bw)}\\
%      &\leq C \abs{\bu + t\bw}^{r-1} + (\lambda_1 + C)\abs{\bu + t\bw}\\
%      &\leq 2^{2-r}C (\abs{\bu}^{r-1} + t^{r-1} \abs{\bw}^{r-1}) + (\lambda_1 + C)(\abs{\bu} + t\abs{\bw})\\
%      &\leq 2^{2-r}C (\abs{\bu}^{r-1} + \abs{\bw}^{r-1}) + (\lambda_1 + C)(\abs{\bu} + \abs{\bw}).
%    \end{align*}
%    The map $[0,1] \ni t \mapsto \abs{\bL(t)}$ is therefore uniformly bounded by a function belonging $L^s(\Omega)$. By Lebesgue's dominated convergence theorem and the continuity of $\phi_1$, we thus get that $\bL$ is continuous and so $L$ is continuous. In other words, $\bLambda_{0,1}$ is hemicontinuous.

%    \medskip
%    \noindent \ul{Monotonicity.} Let $\bv,\bw\in\bV_0$. Writing $\bar \bv = \bv + \bu_\perp$ and $\bar\bw = \bw +\bu_\perp$, we have
%    \begin{align*}
%      \ap{\bLambda_{0,1}(\bv) - \bLambda_{0,1}(\bw),\bv-\bw} &= \int_\Omega ( \phi_1(\abs{\bar \bv}^2) \bar\bv - \phi_1(\abs{\bar \bw}^2) \bar\bw ) \cdot (\bar \bv - \bar \bw)\\
%      &= \int_\Omega \phi_1(\abs{\bar \bv}^2) (\bar\bv - \bar\bw) \cdot (\bar \bv - \bar \bw) + \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot (\bar \bv - \bar \bw)\\
%      &= \int_\Omega \phi_1(\abs{\bar \bv}^2) \abs{\bar\bv - \bar\bw}^2\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot (\bar \bv - \bar \bw)\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot \bar \bv\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) (\abs{\bar\bv}^2 - \abs{\bar \bw}^2)\\
%      &\quad - \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \abs{\bar\bv}^2\\
%      &> \int_\Omega \phi_1(\abs{\bar \bv}^2) \abs{\bar\bv - \bar\bw}^2\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot (\bar \bv - \bar \bw)\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot \bar \bv\\
%      &\quad - \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \abs{\bar\bv}^2\\
%      &= \int_\Omega \phi_1(\abs{\bar \bv}^2) \abs{\bar\bv - \bar\bw}^2\\
%      &\quad - \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot (\bar \bw - \bar \bv)\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) (\bar\bw-\bar\bv) \cdot \bar \bv\\
%      &= \int_\Omega \phi_1(\abs{\bar \bv}^2) \abs{\bar\bv - \bar\bw}^2\\
%      &\quad - \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \abs{\bar \bw - \bar \bv}^2\\
%      &= \frac12 \int_\Omega ( \phi_1(\abs{\bar \bv}^2) + \phi_1(\abs{\bar \bv}^2) ) \abs{\bar\bv - \bar\bw}^2 \geq 0,
%    \end{align*}
%    so that, overall,
%    \begin{equation*}
%      \ap{\bLambda_{0,1}(\bv) - \bLambda_{0,1}(\bw),\bv-\bw} > 0.
%    \end{equation*}
%    Hence $\bLambda_{0,1}$ is strictly monotone. The strict monotonicity stems from the fact that $\phi_1$ is assumed to be strictly increasing.
%  \end{proof}

% \begin{lem}
%   Suppose that $\blambda_1 \preccurlyeq \blambda_2$. The operator $\bLambda_{0,21}$ is maximal.
% \end{lem}

% We thus have shown the existence part of Theorem \ref{thm:wp-1-less-than-2}. The uniqueness part follows from the following lemma:
% \begin{lem}
%   Suppose that $\blambda_1 \preccurlyeq \blambda_2$. The operator $\bLambda_0$ is strongly monotone, that is, there exists $c > 0$ such that
%   \begin{equation*}
%     \ap{\bLambda_{\bv} - \bLambda_{\bw},\bv - \bw} \geq c \norm{\bv - \bw}^2 \quad \text{for all $\bv,\bw\in \bV_0$ and all $\bLambda_{\bv} \in \bLambda_0(\bv)$ and $\bLambda_{\bw} \in \bLambda_0(\bw)$}.
%   \end{equation*}
% \end{lem}
% The uniqueness part from \ref{thm:wp-1-less-than-2} is thus proved. Indeed, if two different solutions to Problem \eqref{eq:weak-form-V0} existed, then the strong monotonicity of $\bLambda_0$ would be violated.



% \section{Single-valued approximation}
% \label{sec:single-valued-approx}

% The question is now to check whether $\bF_*$ satisfies the hypotheses of the Browder--Minty theorem: boundedness, coercivity, hemicontinuity and strict monotonicity. Because of the presence of the Heaviside-like function $H$ in the operator $\bLambda$, we cannot hope for the hemicontinuity of $G$ to hold. For this reason, we shall approximate \eqref{eq:weak-reduced} by a continuous problem.

% Let $H^\e\:\R\to\R$ be a smooth approximation of $H$ converging pointwise to $H$ as the parameter $\e>0$ tends to $0$ and such that $H^\e(1) = h$ (cf. \eqref{eq:heaviside}) for all $\e>0$. For example, if $h=\tfrac12$ then $H^\e$ can be chosen to be the cumulative distribution function of the normal distribution with mean~$1$ and variance $1/\e$. Using from now on upperscripts $\e$ to indicate operators related to the smooth problem, we can write the approximated weak problem, corresponding to \eqref{eq:weak-reduced}: find $\bu^\e\in V^0$ such that
% \begin{equation}
%   \label{eq:weak-reduced-epsilon}
%   \ap{\bF_*^\e(\bu^\e),\bvarphi}_{s,r} = \ap{\bff,\bvarphi}_{s,r} \quad \text{for all $\bvarphi \in V^0$}.
% \end{equation}

% We have the following result:
% \begin{thm}[well-posedness of smooth problem]
%   \label{thm:well-posed-epsilon}
%   Let $\e>0$. There exists a unique $\bu^\e \in V^0$ such that \eqref{eq:weak-reduced-epsilon} holds.
% \end{thm}
% The proof of Theorem \ref{thm:well-posed-epsilon} follows directly from the four lemmas below and the Browder--Minty theorem applied to $\F_*^\e$.

% \begin{lem}[boundedness]
%   Let $\e>0$ and write $S_0$ the unit sphere in $V^0$. The operator $F_*^\e$ is bounded, that is,
%   \begin{equation*}
%     \sup_{\bu \in S_0} \norm{F_*^\e(\bu)}_{L^s(\Omega)} + \norm{F_*^\e(\bnull)}_{L^s(\Omega)} < \infty.
%   \end{equation*}
% \end{lem}

% \begin{lem}[coercivity]
%   Let $\e>0$. The operator $F_*^\e$ is coercive, that is,
%   \begin{equation*}
%     \frac{\ap{F_*^\e(\bu),\bu}_{s,r}}{\norm{\bu}_{L^{r}(\Omega)}} \to \infty \quad \text{as $\norm{\bu}_{L^{r}(\Omega)} \to \infty$}.
%   \end{equation*}
% \end{lem}

% \begin{lem}[hemicontinuity]
%   Let $\e>0$. The operator $F_*^\e$ is hemicontinuous, i.e., the map
%   \begin{equation*}
%     t \mapsto F_*^\e(\bu + t\bv)
%   \end{equation*}
%   is continuous at all $t\in[0,1]$ for all $\bu,\bv \in V^0$.
% \end{lem}

% \begin{lem}[strict monotonicity]
%   Let $\e>0$. The operator $F_*^\e$ is strongly monotone, that is, there exists $C>0$ such that
%   \begin{equation*}
%     \ap{F_*^\e(\bu) - F_*^\e(\bv),\bu - \bv}_{s,r} \geq C\norm{\bu - \bv}_{L^{r}(\Omega)}^2 \quad \text{for all $\bu,\bv\in V^0$}.
%   \end{equation*}
%   In particular, it is strictly monotone.
% \end{lem}


% We shall now show that if $(\bu^\e)_\e \subset V^0$ is a sequence of solutions to \eqref{eq:weak-reduced-epsilon}, then there exists a subsequence of $(\bu_\e)_\e$, still denoted by $(\bu_\e)_\e$, converging to some $\bu\in V^0$ which is solution to \eqref{eq:weak-reduced}.

% \subsection{Browder's theorem}
% \label{sec:browder-thm}

% To show existence of our nonlinear problem we will use the following multivalued extension of the Browder--Minty theorem, due to Browder \comment{referenza: Nonlinear Maximal Monotone Operators in Banach Space} and which we shall therefore refer to as Browder's theorem:
% \begin{thm}[Browder]
%   Let $X$ be a real, separable, reflexive Banach space and let $X^*$ be its dual. Let $T_1$ be a single-valued operator from $X$ to $X^*$ which is bounded, coercive, hemicontinuous and monotone. Let furthermore $T_2$ be a multivalued operator from $X$ to $2^{X^*}$ with $0\in \dom T_2$ which is maximal monotone. Then, the operator $T := T_1 + T_2$ is surjective, i.e.,
%   \begin{equation}
%     \forall\, y\in X^*,\, \exists\, x\in X,\; T(x) = y.
%   \end{equation}
% \end{thm}
% We need to identify the space $X$ and the operator $T$ (and thus $T_1$ and $T_2$) in our setting. To this end, let us introduce the notation $V^0$ for the subset of $L^{r}(\Omega)$ of elements with zero divergence, that is, $\bu\in V^0$ if and only if $\bu \in L^{r}(\Omega)$ and $\ap{\bgrad \psi,\bu}_{s,r} = 0$ for all $\psi\in W^{1,s}(\Omega)$. We show the two lemmas below:
% \begin{lem}
%   \label{lem:bdry-V0}
%   There exists a unique $\bu_*\in L^r(\Omega) \setminus V^0$ such that
%   \begin{equation*}
%     \ap{\bgrad \psi,\bu_*}_{s,r} = -\ap{q,\psi}_{s,r} + \int_{\p\Omega} b\psi \quad \text{for all $\psi\in W^{1,s}(\Omega)$}.
%   \end{equation*}
% \end{lem}
% \begin{proof}
%   \comment{da scrivere, seguire la proposizione 3.1 in AFM.}
% \end{proof}
% \begin{lem}
%   The weak formulation \eqref{eq:weak-form-main} is equivalent to the following problem: find $\bu\in V^0$ such that there exists $\bphi_* \in \bF(\bu+\bu_*)$ satisfying
%   \begin{equation*}
%     \ap{\bphi_*,\bvarphi}_{s,r} = \ap{\bff,\bvarphi}_{s,r} \quad \text{for all $\bvarphi \in V^0$},
%   \end{equation*}
%   where $\bu_*$ is given by Lemma \ref{lem:bdry-V0}.
% \end{lem}
% \begin{proof}
%   \comment{da scrivere, seguire la proposizione 3.2 in AFM.}
% \end{proof}
% Hence the space $X$ and the operator $T$ in Browder's theorem identify in our case with $V^0$ and $\bF_* \: V^0 \to (V^0)^* \sim L^s(\Omega)$, respectively, where
% \begin{equation*}
%   \bF_*(\bu) = \bF(\bu + \bu_*) = \bLambda(\bu + \bu_*)\,(\bu + \bu_*) \quad \text{for all $\bu \in L^{r}(\Omega)$},
% \end{equation*}
% where again $\bu_*$ is as in Lemma \ref{lem:bdry-V0}. Our problem in weak formulation finally reduces to finding $\bu\in V^0$ such that there exists $\bphi_* \in \bF_*(\bu)$ with
% \begin{equation}
%   \label{eq:weak-reduced}
%   \ap{\bphi_*,\bvarphi}_{s,r} = \ap{\bff,\bvarphi}_{s,r} \quad \text{for all $\bvarphi \in V^0$}.
% \end{equation}
% We note from \eqref{eq:multiv-heaviside-law} that $\bF_*$ can be written as the sum of a single-valued operator, namely
% \begin{equation*}
%   \bF_*^1(\bu) := \bF_1(\bu + \bu_*),
% \end{equation*}
% and a multivalued operator, namely
% \begin{equation*}
%   \bF_*^2(\bu) := \bbH(\abs{\bu + \bu_*}^2) (\bF_2(\bu + \bu_*) - \bF_1(\bu + \bu_*)).
% \end{equation*}
% In Browder's theorem we thus identify $T_1$ and $T_2$ with $\bF_*^1$ and $\bF_*^2$, respectively.

% Since obviously $\bnull \in \dom \bF_*^2$, in order to use Browder's theorem we are left with showing that $\bF_*^1$ is bounded, coercive, hemicontinuous and monotone, and that $\bF_*^2$ is maximal monotone, which we do in the following lemmas.
% \begin{lem}[boundedness]
%   Write $S^0$ the unit sphere in $V^0$. The operator $\bF_*^1$ is bounded, that is,
%   \begin{equation*}
%     \sup_{\bu \in S_0} \norm{\bF_*^1(\bu)}_{L^s(\Omega)} + \norm{\bF_*^1(\bnull)}_{L^s(\Omega)} < \infty.
%   \end{equation*}
% \end{lem}

% \begin{lem}[coercivity]
%   The operator $\bF_*^1$ is coercive, that is,
%   \begin{equation*}
%     \frac{\ap{\bF_*^1(\bu),\bu}_{s,r}}{\norm{\bu}_{L^{r}(\Omega)}} \to \infty \quad \text{as $\norm{\bu}_{L^{r}(\Omega)} \to \infty$}.
%   \end{equation*}
% \end{lem}

% \begin{lem}[hemicontinuity]
%   The operator $\bF_*^1$ is hemicontinuous, i.e., the map
%   \begin{equation*}
%     t \mapsto \bF_*^1(\bu + t\bv)
%   \end{equation*}
%   is continuous at all $t\in[0,1]$ for all $\bu,\bv \in V^0$.
% \end{lem}

% \begin{lem}[monotonicity]
%   The operator $\bF_*^1$ is strongly monotone, that is, there exists $C>0$ such that
%   \begin{equation*}
%     \ap{\bF_*^1(\bu) - \bF_*^1(\bv),\bu - \bv}_{s,r} \geq C\norm{\bu - \bv}_{L^{r}(\Omega)}^2 \quad \text{for all $\bu,\bv\in V^0$}.
%   \end{equation*}
%   In particular, it is monotone.
% \end{lem}

% \begin{lem}[maximal monotonicity]
%   The operator $\bF_*^2$ is maximal monotone, that is, it is monotone and the operator $\bs{I} + \alpha \bF_*^2$ is surjective for all $\alpha>0$.
% \end{lem}


% which means that we would need to choose an additional law between the velocity field and the pressure field holding in $\Gamma(\bu)$. To avoid this, we impose that
% \begin{equation}\label{eq:gamma-cond}
%   \text{$\Gamma(\bu)$ is $(d-1)$-dimensional},
% \end{equation}
% which in particular implies that $\Gamma(\bu) = \overline\Omega_1(\bu) \cap \overline\Omega_2(\bu)$. We decompose the velocity field $\bu$ as
v% \begin{equation}\label{eq:u-decomp}
% \bu = \bu_1 + \bu_2,
% \end{equation}
% where, for $i\in\{1,2\}$, we define
% \begin{equation}
%   \bu_i = \bu \chi_{\overline \Omega_i(\bu)\setminus\Gamma(\bu)} + \tfrac12 \bu \chi_{\Gamma(\bu)},
% \end{equation}
% where $\chi_A$ stands for the characteristic function of any set $A$. Note that $\bu_1 = \bu_2$ on $\Gamma(\bu)$. We choose the coupled law $\bF$ as
% \begin{equation}\label{eq:F-coupled}
%   \bF = \bF_1\chi_{\Omega_1(\bu)} + \bF_2\chi_{\Omega_2(\bu)},
% \end{equation}
% which gives, for $i\in\{1,2\}$,
% \begin{equation}
%   \bF(\bu) = \bF_1(\bu_1 + \bu_2)\chi_{\Omega_1(\bu)} + \bF_2(\bu_1 + \bu_2)\chi_{\Omega_2(\bu)} = \bF_i(\bu_i) \quad \text{on $\Omega_i(\bu)$},
% \end{equation}
% and thus, Problem \eqref{eq:div-q}--\eqref{eq:no-flux-cond} becomes, if we ignore for now the interface $\Gamma(\bu)$,
% \begin{equation}\label{eq:main}
%   \begin{cases}
%     \dive \bu_i = q & \text{on $\Omega_i(\bu)$},\\
%     \bF_i(\bu_i) = - \bgrad p + \rho \bf & \text{on $\Omega_i(\bu)$},\\
%     \bu_i \cdot \bn = 0 & \text{on $\p\Omega_i(\bu) \cap \Omega$}.
%   \end{cases}
% \end{equation}
% To close the problem \eqref{eq:main} we now need to get interface conditions, in addition to \eqref{eq:gamma-cond}. Analogously to \eqref{eq:u-decomp}, we decompose the pressure as $p = p_1 + p_2$. The definitions of $\bu_1$, $\bu_2$, $p_1$ and $p_2$ suggest that we should impose $\bu_1=\bu_2$ and $p_1=p_2$ on $\Gamma(\bu)$. We shall relax these conditions slightly on the velocity fields $\bu_1$ and $\bu_2$ by only imposing normal and tangent conditions:
% \begin{equation}\label{eq:interface-cond}
%   \begin{cases}
%     \bu_1 \cdot \bnu = \bu_2 \cdot \bnu,\\
%     \bcurl \bu_1 \times \bnu = \bcurl \bu_2 \times \bnu,\\
%     p_1 = p_2,
%   \end{cases}
%   \quad \text{on $\Gamma(\bu)$},
% \end{equation}
% where $\bnu$ is the outward normal unit vector of $\p\Omega_1$. \comment{[Se ho capito bene, Beavers-Joseph danno condizioni nel caso di un'interfaccia Darcy-Stokes (visto che fanno intevenire il tensore delle tensioni). Nel caso di un'interfaccia generale, per esempio tra Darcy e Darcy-Forchheimer, le condizioni sul curl sopra forse sono più adeguate?]} Our problem of interest in this paper is thus given by \eqref{eq:main}-\eqref{eq:interface-cond} together with the condition \eqref{eq:gamma-cond}.

% \section{The case of two Darcy laws}

% By linearity in this case of the law \eqref{eq:relation-u-p} in the velocity field $\bu$ we get that $\bF$ in \eqref{eq:F-coupled} can written as
% \begin{equation}
%   \bF(\bu) = \mu \bK^{-1}(\bu) \bu,
% \end{equation}
% where the velocity-dependent permeability tensor $\bK(\bu)$ is given by
% \begin{equation}\label{eq:K-darcy-darcy}
%   \bK(\bu) = \bK_1 \chi_{\Omega_1(\bu)} + \bK_2 \chi_{\Omega_2(\bu)}.
% \end{equation}
% We are therefore looking at the following Darcy model:
% \begin{equation}\label{eq:darcy-darcy}
%   \begin{cases} \dive \bu = q,\\ \bK^{-1}(\bu) \bu = -\bgrad p + \rho \bf,\end{cases}
% \end{equation}
% where $\bK(\bu)$ is as in \eqref{eq:K-darcy-darcy}.


% \section{One-dimensional case}
% \label{sec:1d}

% In one dimension, the domain $\Omega$ reduces to an interval. Without loss of generality, we choose $\Omega = (-1,1)$. If we impose $\Gamma(u)$ to be $0$-dimensional, we have $\Gamma(u) = \{\gamma_1(u),\gamma_2(u),\dots\}$ for some family $\{\gamma_k(u)\}_k \subset [-1,1]$. Problem \eqref{eq:main} writes
% \begin{equation}\label{eq:main-1d}
%   \begin{cases}
%     u_i' = q,\\
%     F_i(u_i) = -p' + \rho f,\\
%     u(0) = u(1) = 0,
%   \end{cases}
%   \quad \text{on $\Omega_i(u)$}.
% \end{equation}

% Let us suppose that there exists a solution $(u,p)$. Then, given the boundary conditions, we have
% \begin{equation}
%   \begin{cases}
%     u_1(x) = Q(x) & \text{for all $x\in\Omega_1(u)$},\\
%     u_2(x) = Q(x) & \text{for all $x\in\Omega_2(u)$},
%   \end{cases}
% \end{equation}
% where $Q(x) = \int_{-1}^x q(y) \d y$ for $x\in(-1,1)$ is continuous. We therefore get that
% \begin{equation}
%   \begin{gathered}
%     \Omega_1(u) = \{ x \in (-1,1) \st \abs{Q(x)} < \bar u\}, \quad \text{and} \quad \Omega_2(u) = \{ x \in (-1,1) \st \abs{Q(x)} > \bar u\},\\
%     \Gamma(u) = \{ x \in (-1,1) \st \abs{Q(x)} = \bar u\}.
%   \end{gathered}
% \end{equation}
% We notice that to ensure that $\Gamma(u)$ be $0$-dimensional, we need to choose $q$ and $\bar u$ in such a way that $\abs{Q}$ is almost everywhere different from $\bar u$. For example, we cannot have $Q(a) = \bar u$ for some $a\in(-1,1)$ and then $q(x) = 0$ for all $x\in[a,b]$ with some $b\in(a,1)$.

% \begin{ex}
%   Let us give two examples:
%   \begin{enumerate}
%     \item Choose $q \equiv 0$. Then, $Q \equiv 0$ and since $\bar u > 0$ we have $\Gamma(u) = \Omega_2(u) = \emptyset$ and $\Omega_1(u) = \Omega = (-1,1)$.
%     \item Choose the sigmoid function
%     \begin{equation}
%       q(x) = -\frac12 + \frac{1}{1+e^{-x}} \quad \text{for all $x\in(-1,1)$.}
%     \end{equation}
%     Since $q(x) = 0$ only for $x = 0$, we are safe to say that $\Gamma(u)$ is $0$-dimensional. We know that $\max_{(-1,1)} |Q| = \log(1+e)- 1/2 - \log 2 =: q_*>0$ is achieved at $0$ and we know that, as required, $Q(1) = 0$. Therefore,
%     \begin{equation}
%       \begin{cases}
%         \Gamma(u) = \Omega_2(u) = \emptyset,\; \Omega_1(u) = (-1,1) & \text{if $\bar u > q_*$},\\
%         \Gamma(u) = \{0\},\; \Omega_1(u) = (-1,1),\; \Omega_2(u) = \emptyset & \text{if $\bar u = q_*$},\\
%         \Gamma(u) = \{a,b\},\; \Omega_1(u) = (-1,a) \cup (b,1),\; \Omega_2(u) = (a,b) & \text{if $\bar u < q_*$},
%       \end{cases}
%     \end{equation}
%     where $a = \inf Q^{-1}(\bar u)$ and $b = \sup Q^{-1}(\bar u)$.
%   \end{enumerate}
% \end{ex}

% \comment{[Mi sembra che dati i calcoli sopra il caso 1d sia independente dalla scelta di $F$. In dimensione superiore non sarà sicuramente più il caso.]}

% \section{Well-posedness in dimension one}

% We define the (nonlinear) operator $\Lambda \: L^2(\Omega) \to L^2(\Omega)$ by
% \begin{equation}
%   \Lambda(u) = \lambda_1u + (\lambda_2-\lambda_1) H_{\bar u} \circ u\, u \quad \text{for all $u\in L^2(\Omega)$},
% \end{equation}
% where $H_{\bar u}\: \R \to \R_{\geq 0}$ is given for all $a\in \R$ by
% \begin{equation}
%   H_{\bar u}(a) = \begin{cases} 0 & \text{if $\abs{a} < \bar u$},\\ \frac12 & \text{if $\abs{a} = \bar u$},\\ 1 & \text{if $\abs{a} > \bar u$},\end{cases}
% \end{equation}
% and $\lambda_i\:\Omega\to \R_{\geq 0}$ are inverse permeabilities. The weak formulation of our problem can therefore be rewritten as
% \begin{equation}
%   \begin{gathered}
%     \ap{\Lambda(u),\varphi}_{L^2(\Omega)} + \ap{p',\varphi}_{L^2(\Omega)} = \ap{\rho f,\varphi}_{L^2(\Omega)} \quad \text{for all $\varphi \in L^2(\Omega)$},\\
%     \ap{u,\psi'}_{L^2(\Omega)} = - \ap{q,\psi}_{L^2(\Omega)} \quad \text{for all $\psi \in H^1(\Omega)$}.
%   \end{gathered}
% \end{equation}
% We can show that the problem of finding $(u,p) \in L^2(\Omega)\times H^1(\Omega)$ such that the above equation hold is equivalent to finding $u\in V$ such that
% \begin{equation}\label{eq:weak-1d}
%   \ap{G(u),\varphi}_{L^2(\Omega)} := \ap{K(u+v^*),\varphi}_{L^2(\Omega)} = \ap{\rho f,\varphi}_{L^2(\Omega)},
% \end{equation}
% where $v^*$ is the unique element of $L^2(\Omega)$ satisfying
% \begin{equation}
%   \ap{v^*,\psi'}_{L^2(\Omega)} = - \ap{q,\psi}_{L^2(\Omega)} \quad \text{for all $\psi \in H^1(\Omega)$},
% \end{equation}
% and
% \begin{equation}
%   V = \{ v \in L^2(\Omega) \st \forall\, \psi \in H^1(\Omega),\, \ap{v,\psi'}_{L^2(\Omega)} = 0 \}.
% \end{equation}
% Thanks to \eqref{eq:weak-1d}, the existence of a solution to our problem would stem directly from the surjectivity of the operator $G\: L^2(\Omega) \to L^2(\Omega)$ defined by
% \begin{equation}
%   G(u) = \lambda_1(u+v^*) + (\lambda_2-\lambda_1) H_{\bar u} \circ (u+v^*)\, (u+v^*) \quad \text{for all $u\in L^2(\Omega)$}.
% \end{equation}
% The nonlinearity of $G$ (coming from the jump function $H_{\bar u}$) does not allow us to use the Lax--Milgram theorem. Instead, we shall use the Browder--Minty theorem, which generalizes the former to nonlinear operators. We recall it here:
% \begin{thm}[Browder--Minty]
%   A bounded, coercive, hemicontinuous, monotone operator $T$ from a real, separable, refexive Banach space $X$ into its dual $X^*$ is surjective, i.e.,
%   \begin{equation}
%     \forall\, f\in X^*,\, \exists\, u\in X,\; T(u) = f.
%   \end{equation}
% \end{thm}

% The operator $G$ is easily shown to be bounded and coercive. However, it is not hemicontinuous (again because of $H_{\bar u}$). (It is also probably not monotone.) To overcome this, let us approximate our problem by smoothing $H_{\bar u}$, and thus the operators $\Lambda$ and $G$, as follows:
% \begin{equation}
%   H_{\bar u}^\e(a) = \begin{cases} 0 & \text{if $|a| < \bar u - \e$},\\ \sigma^\e(a) & \text{if $-\bar u - \e < a < -\bar u + \e$ or $\bar u - \e < a < \bar u + \e$},\\ 1 & \text{if $|a| > \bar u + \e$}, \end{cases}
% \end{equation}
% where $\sigma^\e\:\R\to\R_{\geq 0}$ is a smooth function such that $H_{\bar u}^\e$ is smooth and
% \begin{equation}
%   \sigma^\e(\bar u) = \sigma^\e(-\bar u) = \tfrac12, \quad \sigma^\e(-\bar u - \e) = \sigma^\e(\bar u + \e) = 1 \quad \text{and} \quad \sigma^\e(-\bar u + \e) = \sigma^\e(\bar u - \e) = 0.
% \end{equation}
% The resulting operator $G^\e$ should be continuous and monotone.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "interface_master"
%%% End:



==> interface2.tex <==
\section{Proposed model}
\label{sec:proposed-model}

We identify our fracture network with an open, bounded connected set $\Omega \subset \R^d$ with Lipschitz boundary filled with a fluid of constant density $\rho \equiv 1$. Thus, mass conservation in $\Omega$ reads
\begin{equation}
  \label{eq:div-q}
  \dive \bu = q,
\end{equation} 
where $\bu\: \Omega \to \R^d$ is the unknown velocity of the fluid and $q\: \Omega \to \R$ a given source term allowing, for instance, for fluid mass to be exchanged between the fractures and the surrounding porous medium. Writing $\p\Omega$ the boundary of $\Omega$, let $\Sigma_{\mt{v}},\Sigma_{\mt{p}} \subset \p\Omega$ be relatively open and such that $\p\Omega = \overbar{\Sigma_{\mt{v}} \cup \Sigma_{\mt{p}}}$ and $\Sigma_{\mt{v}} \cap \Sigma_{\mt{p}} = \emptyset$. To \eqref{eq:div-q} we add the following boundary conditions:
\begin{equation}
  \label{eq:neumann-cond}
  \begin{cases}
    \bu \cdot \bn = u_0 & \text{on $\Sigma_{\mt{v}}$},\\
    p = p_0 & \text{on $\Sigma_{\mt{p}}$},
  \end{cases}
\end{equation}
where $p\:\Omega \to \R$ is the unknown pressure of the fluid and $\bn$ is the outward normal unit vector of $\p\Omega$. Here, $u_0: \Sigma_{\mt{v}} \rightarrow \R$ and $p_0\:\Sigma_{\mt{p}}\to\R$ are given functions setting the conditions on the boundary of $\bu$ and $p$, respectively. Note that we are denoting maps on $\Omega$ and their traces on the boundary $\p\Omega$ by the same notation.  

\subsection{Velocity-pressure law}
\label{sec:vel-press-law}

Typically, one couples \eqref{eq:div-q} and \eqref{eq:neumann-cond} with a relation, or law, between the velocity field $\bu$ and the pressure field $p$ via some operator $\bLambda$:
\begin{equation}
  \label{eq:relation-u-p}
  \bLambda(\bu) = -\bgrad p + \bff,
\end{equation}
where $\bff$ is a given body force (e.g., gravity). Examples of laws $\bLambda$ relating velocity and pressure via \eqref{eq:relation-u-p} are
\begin{equation}\label{eq:F-ex}
  \begin{gathered}
    \bLambda_\mt{S}(\bu) = -\bLap \bu, \quad \bLambda_\mt{D}(\bu) = \bK^{-1} \bu,\\
    \quad \bLambda_\mt{B}(\bu) = -\bLap \bu + \bK^{-1} \bu, \quad \bLambda_\mt{DF}(\bu) = \bK^{-1} \bu + \alpha\norm{\bu}^{r-2}\bu,
  \end{gathered} 
\end{equation}
where $\bK \: \Omega \to \R^{d\times d}$ is the permeability tensor and $\alpha\geq 0$ and $r\in\R_{\geq 2}$ some parameters. Choosing $\bLambda_\mt{S}$ gives Stokes' equation, $\bLambda_\mt{D}$ gives Darcy's equation, $\bLambda_\mt{B}$ gives Brinkman's equation and $\bLambda_\mt{DF}$ gives the generalized Darcy--Forchheimer equation (which simplifies into the common Darcy--Forchheimer when $r=3$).

The study of \eqref{eq:div-q} and \eqref{eq:neumann-cond} together with a law of the form \eqref{eq:relation-u-p} is very well-documented in the literature. \comment{referenze...} To the authors' knowledge, a known issue that has not yet found a documented answer is the case when one needs to choose a combination of laws such as those given as examples in \eqref{eq:F-ex}, rather than a single one, i.e., when one needs to couple different velocity-pressure laws according to some validity criterion which selects the better-adapted law. This criterion should depend on the speed regime (or Reynolds number) of the flow. For example, where the Reynolds number is low Darcy's law $\bLambda_\mt{D}$ may be preferred, whereas where it is high Stokes' equation $\bLambda_\mt{S}$ might be chosen instead. For this reason, in this paper we consider the case where we need to choose from two laws $\bLambda_1$ and $\bLambda_2$ according to some threshold speed $\bar u > 0$. In this setting, the law operator in \eqref{eq:relation-u-p} takes the form
\begin{equation}
  \label{eq:law-jump}
  \bLambda(\bu) =
  \begin{cases}
    \bLambda_1(\bu) & \text{whenever $\norm{\bu} < \bar u$},\\
    \bLambda_2(\bu) & \text{whenever $\norm{\bu} > \bar u$}.
  \end{cases}
\end{equation}
Being able to impose a law at the interface $\{\norm{\bu} = \bar u\}$ is out of the scope of this paper---we will therefore consider our problem solved whenever we find a pressure field and a velocity field such that \eqref{eq:div-q}--\eqref{eq:relation-u-p} and \eqref{eq:law-jump} hold. This summarizes as finding functions $\bu$ and $p$ solving
\begin{equation}
  \label{eq:main-model}
  \begin{cases}
    \dive \bu = q & \text{on $\Omega$},\\
    \bLambda(\bu) = -\grad p + \bff & \text{on $\Omega$},\\
    \bu\cdot\bn = u_0  & \text{on $\Sigma_{\mt{v}}$},\\
    p = p_0  & \text{on $\Sigma_{\mt{p}}$},
  \end{cases}
\end{equation}
where $\bLambda$ is as in \eqref{eq:law-jump}. Clearly, when $\bLambda_1\neq\bLambda_2$, this choice of adaptable law introduces a discontinuity at $\norm{\bu} = \bar u$ which we shall treat carefully when studying existence of solutions. We will complete the strong formulation \eqref{eq:main-model} in Section \ref{sec:assu-vel-press}, where a multivalued weak setting will be introduced so as to be able to treat the interface without imposing any given law on it.

\begin{rem}
  Whenever the boundary piece $\Sigma_{\mt{p}}$ is such that $\mt{Vol}^{d-1}(\Sigma_{\mt{p}}) = 0$, it is classical to add to \eqref{eq:main-model} a constraint on the average of the pressure field:
\begin{equation}
  \label{eq:pressure-average}
  \frac{1}{\abs{\Omega}}\int_\Omega p = \sigma,
\end{equation}
for some $\sigma\in\R$. Indeed, this is often required to ensure uniqueness of the pressure field satisfying Problem \eqref{eq:main-model} when $\bLambda$ is a classical continuous law. Similarly we will impose \eqref{eq:pressure-average} whenever $\mt{Vol}^{d-1}(\Sigma_{\mt{p}}) = 0$, so that our problem in this case becomes: find functions $\bu$ and $p$ such that 
\begin{equation*}
  \begin{cases}
    \dive \bu = q & \text{on $\Omega$},\\
    \bLambda(\bu) = -\grad p + \bff & \text{on $\Omega$},\\
    \bu\cdot\bn = u_0  & \text{on $\p\Omega$},
  \end{cases}
\end{equation*}
under the constraint \eqref{eq:pressure-average}, where $\bLambda$ is given in \eqref{eq:law-jump}. For ease of discussion, however, we will often silence \eqref{eq:pressure-average} and only refer to \eqref{eq:main-model} as being our problem, even when $\mt{Vol}^{d-1}(\Sigma_{\mt{p}}) = 0$; it will nevertheless be naturally encoded in our weak formulation.
\end{rem}

We focus in this paper on Darcy-like operator laws, that is, laws involving no derivatives of the velocity field, so that we need to exclude Stokes' and Brinkman's equations as admissible examples. Under some additional conditions (depending in particular on the direction of the jump between laws $\bLambda_1$ and $\bLambda_2$ at the interface), we show existence of solutions via the study of an energetic formulation of \eqref{eq:main-model}. Indeed, we are able to define an energy functional on the space of velocity fields whose minimizers satisfy \eqref{eq:main-model}. Although we have uniqueness for this energetic formulation, this property does not transfer to \eqref{eq:main-model}---this is natural since we are not imposing what the velocity-pressure law should be on the interface. In order to hope for uniqueness, one should either impose an adequate law on the interface or show that the interface must have zero Lebesgue measure so that it does not play a role in defining weak solutions. As already mentioned, we do not wish to focus on the problem of the interface at this stage and leave it to a later work.

\subsection{Intersecting fractures}

In the case $\Omega$ is composed by multiple intersecting fracture branches, forming thus a
fracture network, we can extend the previous model by including suitable
interface conditions at the intersections. Given $\Omega$ we introduce $\omega^i
\subset \Omega$ to be a fracture branch, with $n_\omega \ni i$ the total number
of branches. Clearly, given two distinct branches $\omega^i$ and $\omega^j$,
with $i\neq j$, we have $\mathring{\omega}^i \cap \mathring{\omega}^j =
\emptyset$ and also that $\overline{\Omega} = \cup_{i =1}^{n_\omega}
\overline{\omega}^i$.

We consider $2 \leq n \leq n_\omega$ fracture branches that meet in an
intersection $\overline{\mathcal{I}} = \cap_{i=1}^n \overline{\omega}^i$, to
complete model \eqref{eq:main-model} in $\mathcal{I}$ we impose the following conditions
\begin{gather}\label{eq:network_cc}
    \sum_{i=1}^n \bu^i \cdot \bn^i = 0
    \quad \text{and} \quad
    p^i = p^j \quad \forall i, j=1, \ldots, n
\end{gather}
where with a superscript $i$ we indicate the corresponding object restricted to
$\omega^i$, and
$\bn^i$ is a unit vector tangent to $\omega^i$ and pointing to
$\mathcal{I}$, in the mono-dimensional case, and in addition normal to $\partial
\omega^i$, in the multi-dimensional case. This condition is frequently used, see
for instance \cite{Alboin2000a,Amir2005,Berrone2013a,Berrone2013}.

The first condition in \eqref{eq:network_cc} is a direct consequence of the conservation of mass at the
intersection, while the second can be derived from each constitutive relation of
the form \eqref{eq:relation-u-p}. These conditions do not put any additional
difficulties in the analysis and are therefore considered only in the numerical
examples.

It is possible to consider more complex conditions that allow pressure and
velocity jump at the intersection, see among others
\cite{Formaggia2012,Boon2018,Berre2020a}. However, since this is
not the main focus we keep the simpler interface condition \eqref{eq:network_cc}.



% In this setting we can write our law operator $\bLambda$ in \eqref{eq:relation-u-p} as a combination of the operators $\bLambda_1$ and $\bLambda_2$ and an additional interface law operator $\bLambda_\Gamma$, such as
% \begin{equation*}
%   \bLambda(\bu) = \bLambda_1(\bu) \chi_{\Omega_1(\bu)} + \bLambda_2(\bu) \chi_{\Omega_2(\bu)} + \bLambda_\Gamma(\bu) \chi_{\Gamma(\bu)},
% \end{equation*}
% where $\chi_A$ is the indicator function of any set $A\subset\R^d$. The choice of the interface law seems to be aribitrary at this point, especially if we expect the interface to be of dimension lower than $d$. We might then be tempted to choose the zero law 
% \begin{equation*}
%   \bLambda_\Gamma(\bu) = \bnull,  
% \end{equation*}
% that is, to impose that the pressure has to satisfy $\bgrad p = \bff$ (and the velocity, by definition, $\abs{\bu} = 1$) on the interface. Another attempt, probably more satisfactory, would be to choose the interface law operator as a convex combination between $\bLambda_1$ and $\bLambda_2$, as in
% \begin{equation}
%   \label{eq:law-convex}
%   \bLambda_\Gamma(\bu) = (1 - \tau) \bLambda_1(\bu) + \tau\bLambda_2(\bu),
% \end{equation}
% for some given $\tau\in[0,1]$, so that, for example, choosing $\tau=\tfrac12$ would mean that the interface law is the arithmetic average of the two ``main'' laws, yielding $\frac12 (\bLambda_1(\bu) + \bLambda_2(\bu)) + \bgrad p = \bff$ on the interface. A natural choice for $\bLambda_\Gamma$ stems from the following formal energetic consideration.

% In this convex combination setting, the law would take the form
% \begin{equation*}
%   \bLambda(\bu) = (1 - H_\tau(\abs{\bu})) \bLambda_1(\bu) + H_\tau(\abs{\bu}) \bLambda_2(\bu),
% \end{equation*}
% where $H_\tau\: \R \to \R$ is the Heaviside-like function defined for all $a\in\R$ by
% \begin{equation}
% \label{eq:heaviside-param}
%   H_\tau(a) =
%   \begin{cases}
%     0 & \text{if $a < 1$},\\
%     \tau & \text{if $a = 1$},\\
%     1 & \text{if $a > 1$}.
%   \end{cases}
% \end{equation}
% Taking a convex combination of the two ``main'' laws as in \eqref{eq:law-convex} within the interface seems to be a plausible choice as it ensures that the interface law operator is somewhat controlled by $\bLambda_1$ and $\bLambda_2$. When $d=1$, in fact, this combination makes sure that $\Lambda_\Gamma$ stays between $\Lambda_1$ and $\Lambda_2$. The issue with \eqref{eq:law-convex} is to decide where on the segment $[0,1]$ we should choose the parameter $\tau$, that is, which law along the convex combination between $\bLambda_1$ and $\bLambda_2$ we should choose. We may actually need to consider a function $\tau\: \Omega \to [0,1]$ as parameter rather than a fixed number; this is in fact the natural setting that emerges from a formal energetic consideration, as we explain below.

%  We cannot answer this point if we do not wish to give ourselves additional apriori knowledge on the interface. In this paper we will circumvent this issue by choosing a multivalued version of \eqref{eq:law-convex}, as described in Section \ref{sec:multiv-setting}.

% \begin{rem}
%   A further possible generalization of \eqref{eq:law-convex} would be to choose the interface law operator as a generic interpolation between $\bLambda_1$ and $\bLambda_2$ parametrized by some $h\in[0,1]$, as in
%   \begin{equation*}
%     \bLambda_\Gamma(\bu) = \bs{I}_h(\bLambda_1(\bu),\bLambda_2(\bu)),
%   \end{equation*}
%   where $(\bs{I}_h)_{h\in[0,1]}$ is a parametrized interpolator satisfying $\bs{I}_0(\ba,\bb) = \ba$ and $\bs{I}_1(\ba,\bb) = \bb$ for all $\ba,\bb\in\R^d$. Choosing $\bs{I}_h(\ba,\bb) = (1 - h) \ba + h\bb$ would recover the convex combination case \eqref{eq:law-convex}, whereas choosing 
%   \begin{equation*}
%     \bs{I}_h(\ba,\bb) =  \abs{\ba}^h\abs{\bb}^{1-h} \left( \frac{(1-h)\ba}{\abs{\ba}} + \frac{h\bb}{\abs{\bb}} \right) \quad \text{or} \quad \bs{I}_h(\ba,\bb) = \left( \frac{1-h}{\abs{\ba}} + \frac{h}{\abs{\bb}} \right)^{-1} \left( \frac{(1-h)\ba}{\abs{\ba}} + \frac{h\bb}{\abs{\bb}} \right)
%   \end{equation*}
%   would give geometric-like or harmonic-like average laws, respectively. We choose not to explore this interpolated interface law in the present paper as it adds significant technical challenges to the convex combination case and we do not wish to study the interface in such depth at this point. We shall leave this issue, together with that of determining the dimensionality of the interface, for a subsequent paper.
% \end{rem}

% \subsection{Formal energetic consideration}
% \label{sec:energetic-cons}

% Suppose that the law operators $\bLambda_1$ and $\bLambda_2$ take the forms
% \begin{equation*}
%   \bLambda_1(\bu) = \phi_1(\abs{\bu}^2)\bu \quad \text{and} \quad \bLambda_2(\bu) = \phi_2(\abs{\bu}^2)\bu,
% \end{equation*}
% where $\phi_1$ and $\phi_2$ are functions with enough regularity for the following consideration to hold. The classical setting is recovered here by taking $\phi_1 \equiv \phi_2 =: \phi$ and consequently $\bLambda_1 = \bLambda_2$. In this case it is known \comment{(referenza Spena-Vacca)} that, when $\phi$ is continuous and nondecreasing, solving \eqref{eq:div-q}--\eqref{eq:relation-u-p} is equivalent to minimizing on an adequate function space the energy
% \begin{equation*}
%   \E(\bu) = \int_\Omega \left( \Phi(\abs{\bu}^2) - \bff \cdot \bu \right),
% \end{equation*}
% where $\Phi$ is any primitive of $\tfrac\phi2$. Indeed, we have that $\E$ is differentiable and convex with gradient $\bgrad \E$ given by
% \begin{equation*}
%   \bgrad \E(\bu) = \phi(\abs{\bu}^2) \bu - \bff = \bLambda(\bu) - \bff,
% \end{equation*}
% so that minimizing $\E$ is equivalent to finding $\bu$ with $\bLambda(\bu) = \bff$, since in this case $\bgrad \E(\bu) =\bnull$. Writing
% \begin{equation*}
%   \D(\bu) = \int_\Omega \Phi(\abs{\bu}^2)
% \end{equation*}
% what is typically referred to as the dissipation functional, we see that $\bLambda(\bu) = \grad \D(\bu)$.

% Following this approach in the general case where we may have $\phi_1 \not\equiv \phi_2$, the corresponding energy and dissipation are
% \begin{equation*}
%   \E(\bu) = \D(\bu) - \int_\Omega \bff\cdot\bu \quad \text{and} \quad \D(\bu) = \int_\Omega \left( \Phi_1(\abs{\bu}^2)\chi_{\Omega_1(\bu)} + \Phi_2(\abs{\bu}^2)\chi_{\Omega_2(\bu)} \right),
% \end{equation*}
% where and $\Phi_1$ and $\Phi_2$ are primitives of $\tfrac{\phi_1}{2}$ and $\tfrac{\phi_2}{2}$ to be chosen appropriately. Setting $\Psi(a) = \Phi_1(a)\chi_{a<1} + \Phi_2(a)\chi_{a>1}$ we can rewrite 
% \begin{equation*}
%   \E(\bu) = \int_\Omega \left( \Psi(\abs{\bu}^2) - \bff\cdot\bu \right) \quad \text{and} \quad \D(\bu) = \int_\Omega \Psi(\abs{\bu}^2).
% \end{equation*}
% We note that $\Psi$ is continuous only provided that $\Phi_1(1) = \Phi_2(1) = 0$. We therefore choose the primitives $\Phi_1$ and $\Phi_2$ to be such that $\Phi_1(1) = \Phi_2(1) = 0$. When $\phi_1$ and $\phi_2$ are continuous and nondecreasing we notice that the Fréchet subdifferential $\p\E$ satisfies
% \begin{equation*}
%   \p\E(\bu) = \begin{cases} \{\phi_1(\abs{\bu}^2)\bu - \bff\} = \{\bLambda_1(\bu) - \bff\}& \text{on $\Omega_1(\bu)$},\\ \{\phi_2(\abs{\bu}^2)\bu - \bff\} = \{\bLambda_2(\bu) - \bff\} & \text{on $\Omega_2(\bu)$}. \end{cases}
% \end{equation*}
% From subdifferential calculus we know that, even when $\E$ is not convex, a function $\bu$ is a local minimizer of $\E$ if and only if $\bnull \in \p\E(\bu)$. This consideration therefore invites us to consider a multivalued setting where the law operator $\bLambda$ is in fact the \emph{set} of operators given by the subdifferential of $\D$:
% \begin{equation*}
%   \bLambda(\bu) = \p\D(\bu).
% \end{equation*}
% This is the setting we choose for the rest of the paper.

% In this case, we also note that when $\phi_1$ and $\phi_2$ are convex and $\phi_1(1) \leq \phi_2(1)$ the energy $\E$ is convex and its subdifferential $\p\E$ is given, as we will prove later, by 
% \begin{align*}
%   \p \E(\bu) &= (1 - \frakH(\abs{\bu}^2)) \phi_1(\abs{\bu}^2) \bu + \frakH(\abs{\bu}^2) \phi_2(\abs{\bu}^2) \bu - \bff\\
%   &= (1 - \frakH(\abs{\bu}^2)) \bLambda_1(\bu) + \frakH(\abs{\bu}^2) \bLambda_2(\bu) - \bff,
% \end{align*}
% where $\frakH \: \R \to 2^{L^\infty(\Omega;[0,1])}$ is defined for all $a\in\R$ as
% \begin{equation}
%   \label{eq:heaviside-multiv}
%   \frakH(a) =
%   \begin{cases}
%     \{0\} & \text{if $a < 1$},\\
%     L^\infty(\Omega;[0,1]) & \text{if $a = 1$},\\
%     \{1\} & \text{if $a > 1$}.
%   \end{cases}
% \end{equation}
% (Within the above curly brackets, $0$ and $1$ stand respectively for the zero and one constant functions, which of course belong to $L^\infty(\Omega;[0,1])$.) 


\section{Mathematical setting}
\label{sec:math-setting}

We give in this section the rigorous mathematical setting; in particular we introduce the assumptions on the underlying law operators as well as the weak formulation of our problem. We shall use the convention to use boldfaced symbols for vectors and vector-valued functions. 

From now on, without loss of generality we take $\bar u$ to be equal to $1$. For a given field $\bu\:\Omega\to \R^d$, we write 
\begin{equation}
  \begin{gathered}
    \Omega_1(\bu) = \{ \bx\in \Omega \st \norm{\bu(\bx)} < 1 \}, \quad \Omega_2(\bu) = \{ \bx\in \Omega \st \norm{\bu(\bx)} > 1\},\\ \Gamma(\bu) = \Omega\setminus (\Omega_1(\bu) \cup \Omega_2(\bu)) = \{\bx\in \Omega \st \norm{\bu(\bx)} = 1 \},
  \end{gathered}
\end{equation}
where $\Gamma(\bu)$ is what we have already referred to as the \emph{interface} (associated with $\bu$). Obviously, the family $\mathcal{C} = \{\Omega_1(\bu),\Omega_2(\bu),\Gamma(\bu)\}$ forms a partition of $\Omega$, we will refer to $\mathcal{C}$ also as the configuration of the problem. We can rewrite these sets in a more compact form as:
\begin{equation*}
  \Omega_1(\bu) = \bu^{-1}(B_1(\bnull)), \quad \Omega_2(\bu) = \bu^{-1}(E_1(\bnull)), \quad \Gamma(\bu) = \bu^{-1}(S_1(\bnull)),
\end{equation*}
where $B_1(\bnull)$ and $S_1(\bnull)$ stand respectively for the unit open ball and unit sphere in $\R^d$ centered at the origin $\bnull$ and $E_1(\bnull) = \R^d\setminus (B_1(\bnull)\cup S_1(\bnull))$. Note that if $\bu$ is not continuous, then $\Omega_1(\bu)$ and $\Omega_2(\bu)$ may not be open.

For all $t\in[1,\infty)$ we will denote by $L^t(\Omega)$ and $W^{1,t}(\Omega)$ the Lebesgue space of measurable functions on $\Omega$ with integrable $r$th power and the first-order Sobolev space associated to $L^t(\Omega)$; we will also write $\bL^t(\Omega)$ in place of $(L^t(\Omega))^d$. As usual, in these spaces, equality between two functions is always intended in the almost-everywhere sense.

\subsection{Assumptions on the velocity-pressure laws}
\label{sec:assu-vel-press}

In the following, the operator laws $\bLambda_1$ and $\bLambda_2$ are assumed to be of the form
\begin{equation}
  \label{eq:law-form}
  \bLambda_1(\bu) = \phi_1(\norm{\bu}^2)\bu \,\chi_{\Omega_1(\bu)} \quad \text{and} \quad \bLambda_2(\bu) = \phi_2(\norm{\bu}^2) \bu \,\chi_{\Omega_2(\bu)},
\end{equation}
where $\chi_A$ is the characteristic function of any set $A\subset\R^d$. The functions $\phi_1,\phi_2\: [0,\infty) \to [0,\infty)$ are continuous and increasing on $[0,1]$ and $[1,\infty)$, respectively. Furthermore, $\phi_2$ satisfies the following assumption: there exist $r\geq 2$ and $c,C>0$ such that
\begin{equation}
  \label{eq:bound-phi2}
   c a^{\frac{r-2}{2}} \leq \phi_2(a) \leq C \left(1+a^{\frac{r-2}{2}}\right) \quad \text{for all $a\geq 1$}.
\end{equation}
The Darcy operator $\bLambda_\mt{D}$ as well as Darcy-Forchheimer $\bLambda_\mt{DF}$ in \eqref{eq:F-ex} fulfil requests \eqref{eq:law-form} and \eqref{eq:bound-phi2}.

\begin{rem}
  This setting where $\bLambda_1$ and $\bLambda_2$ are as in \eqref{eq:law-form} physically restricts us to scalar permabilities. More general laws including tensor permeabilities, as motivated in \comment{Spena-Vacca}, are for instance given by the following:
  \begin{equation*}
    \bLambda_1(\bu) = \phi_1(\blambda_1\bu\cdot\bu)\blambda_1\bu,
  \end{equation*}
and analogously for $\bLambda_2$, where $\blambda_1\in\R^{d\times d}$ is a symmetric positive definite matrix encoding a tensor permeability. Even more general forms are envisageable:
\begin{equation*}
    \bLambda_1(\bu) = \sum_{j=1}^n \phi_{1,j}(\blambda_{1,j}\bu\cdot\bu)\blambda_{1,j}\bu,
  \end{equation*}
where the $\phi_{1,j}$ and $\blambda_{1,j}$ are $n$ different law functions and permeability tensors. We leave these general laws to a future work. We claim that the techniques we use in the present paper for scalar laws should extend to tensor laws without too much difficulty.
\end{rem}

We denote by $s = \tfrac{r}{r-1}$ the conjugate exponent of $r$. Thanks to the continuity of $\phi_1$ and the right-hand inequality in \eqref{eq:bound-phi2}, we observe that the operators $\bLambda_1$ and $\bLambda_2$ map $\bL^r(\Omega)$ into $\bL^s(\Omega)$. Because we allow for any law on the interface, this invites us to consider the multivalued setting where our combined law $\bLambda$ maps $\bL^r(\Omega)$ into the power set $2^{\bL^s(\Omega)}$ and is given by
\begin{equation}
  \label{eq:law-combined}
  \bLambda(\bu) =
  \begin{cases}
    \{\bLambda_1(\bu)\} & \text{on $\Omega_1(\bu)$},\\
    \bL^s(\Omega) & \text{on $\Gamma(\bu)$},\\
    \{\bLambda_2(\bu)\} & \text{on $\Omega_2(\bu)$}.
  \end{cases}
\end{equation}

% Our combined law $\bLambda$ defined in \eqref{eq:multiv-heaviside-law} maps $\bL^r(\Omega)$ to the power set $2^{\bL^s(\Omega)}$. Indeed, let $\bu\in\bL^r(\Omega)$ and $\bLambda_{\bu} \in \bLambda(\bu)$ and write $\tau\in L^\infty(\Omega;[0,1])$ such that $\bLambda_{\bu} = \bLambda(\tau;\bu)$; then, writing $\sigma = \sup_{a\in[0,1]}\phi_1(a)$, which is finite thanks to the continuity of $\phi_1$, and using the right-hand inequality in \eqref{eq:bound-phi2} and the fact that $1 < s \leq r$, we get
% \begin{align*}
%   \norm{\bLambda_{\bu}}_{\bL^s(\Omega)}^s &= \int_{\Omega_1(\bu)} \abs{\phi_1(\abs{\bu}^2)\bu}^s + \int_{\Omega_2(\bu)} \abs{\phi_2(\abs{\bu}^2)\bu}^s + \int_{\Gamma(\bu)} \abs{((1-\tau) \lambda_1 + \tau\lambda_2)\bu}^s\\
%   &\leq \sigma^s \int_{\Omega_1(\bu)} \abs{\bu}^s + 2^{s-1}C^s\int_{\Omega_2(\bu)} \abs{\bu}^s + 2^{s-1}C^s\int_{\Omega_2(\bu)} \abs{\bu}^r  + \max\{\lambda_1,\lambda_2\}^s \int_{\Gamma(\bu)}\abs{\bu}^s\\
%   &\leq \sigma^s \abs{\Omega} + 2^{s-1}C^s\int_{\Omega_2(\bu)} \abs{\bu}^r + 2^{s-1}C^s\int_{\Omega_2(\bu)} \abs{\bu}^r  + \max\{\lambda_1,\lambda_2\}^s \abs{\Omega}\\
%   &\leq 2^sC^s\norm{\bu}_{\bL^r(\Omega)}^r + (\sigma^s + \max\{\lambda_1,\lambda_2\}^s)\abs{\Omega} <\infty.
% \end{align*}


\subsection{Weak formulation}
\label{sec:weak-formulation}

We fix $q\in L^r(\Omega)$, $u_0\in L^{r}(\Sigma_{\mt{v}})$, $p_0\in W^{1-\frac{1}{s},s}(\Sigma_{\mt{p}})$ and $\bff\in \bL^s(\Omega)$. Consider the Sobolev space
\begin{equation*}
  \widetilde W^{1,s}(\Omega) = 
  \begin{cases}
    \left\{ \xi \in W^{1,s}(\Omega) \st \displaystyle \frac{1}{\abs{\Omega}}\int_\Omega \xi = \sigma \right\} & \text{if $\mt{Vol}^{d-1}(\Sigma_{\mt{p}}) = 0$},\\
    \left\{ \xi \in W^{1,s}(\Omega) \st \xi = p_0\; \text{on $\Sigma_{\mt{p}}$} \right\} & \text{if $\mt{Vol}^{d-1}(\Sigma_{\mt{p}}) > 0$},
  \end{cases}
\end{equation*}
where $\mt{Vol}^{d-1}$ stands for the $(d-1)$-dimensional Lebesgue measure. The problem we shall focus on in the rest of the paper is: find $(\bu,p) \in \bL^r(\Omega)\times \widetilde W^{1,s}(\Omega)$ so that there exists $\bLambda_{\bu} \in \bLambda(\bu)$ such that for all $\bvarphi\in \bL^r(\Omega)$ and $\psi\in \widetilde W^{1,s}(\Omega)$ there holds
\begin{equation}
  \label{eq:weak-form-tilde}
  \begin{gathered}
    \int_\Omega \bLambda_{\bu} \cdot \bvarphi = - \int_\Omega \bgrad p \cdot\bvarphi + \int_\Omega \bff\cdot\bvarphi,\\
    \int_\Omega \bgrad \psi\cdot \bu = -\int_\Omega q\psi + \int_{\Sigma_{\mt{v}}} u_0\psi,
  \end{gathered}
\end{equation}
where we recall that $\bLambda$ is given in \eqref{eq:law-combined}. From the linearity of \eqref{eq:weak-form-tilde} with respect to the pressure field, we see that, by setting $\bff_0 = \bff + \bgrad (E p_0)$, with $E: W^{1-\frac{1}{s},s}(\Sigma_{\mt{p}}) \rightarrow W^{1,s}(\Omega)$ the extension operator being the right-inverse of the $W^{1,s}(\Omega)$-trace operator,
and defining the Sobolev space
\begin{equation*}
  W_0^{1,s}(\Omega) = 
  \begin{cases}
    \left\{ \xi \in W^{1,s}(\Omega) \st \displaystyle \int_\Omega \xi = 0 \right\} & \text{if $\mt{Vol}^{d-1}(\Sigma_{\mt{p}}) = 0$},\\
    \left\{ \xi \in W^{1,s}(\Omega) \st \xi = 0\; \text{on $\Sigma_{\mt{p}}$} \right\} & \text{if $\mt{Vol}^{d-1}(\Sigma_{\mt{p}}) > 0$},
  \end{cases}
\end{equation*}
the formulation in \eqref{eq:weak-form-tilde} is equivalent to: find $(\bu,p) \in \bL^r(\Omega)\times W_0^{1,s}(\Omega)$ so that there exists $\bLambda_{\bu} \in \bLambda(\bu)$ such that for all $\bvarphi\in \bL^r(\Omega)$ and $\psi\in W_0^{1,s}(\Omega)$ there holds
\begin{equation}
  \label{eq:weak-form}
  \begin{gathered}
    \int_\Omega \bLambda_{\bu} \cdot \bvarphi = - \int_\Omega \bgrad p \cdot\bvarphi + \int_\Omega \bff_0\cdot\bvarphi,\\
    \int_\Omega \bgrad \psi\cdot \bu = -\int_\Omega q\psi + \int_{\Sigma_{\mt{v}}} u_0\psi.
  \end{gathered}
\end{equation}
We endow $W_0^{1,s}(\Omega)$ with the norm $\norm{\psi}_{W_0^{1,s}(\Omega)} = \norm{\bgrad\psi}_{\bL^s(\Omega)}$ for all $\psi\in W_0^{1,s}(\Omega)$.

Thanks to Riesz's representation theorem, we shall equivalently manipulate functions in $\bL^s(\Omega)$ as elements of $(\bL^r(\Omega))^*$, the dual of $\bL^r(\Omega)$. In particular, this means that, given $\bu\in \bL^r(\Omega)$, operators $\bLambda_{\bu}$ in $\bLambda(\bu)$ will also be seen as maps from $\bL^r(\Omega)$ to $(\bL^r(\Omega))^* \sim \bL^s(\Omega)$. Writing $\ap{\cdot,\cdot}$ the dual mapping on $\bL^s(\Omega)\times \bL^r(\Omega)$, the weak formulation in \eqref{eq:weak-form} of our problem can be restated as follows: find $(\bu,p)\in \bL^r(\Omega)\times W_0^{1,s}(\Omega)$ so that there exists $\bLambda_{\bu} \in \bLambda(\bu)$ such that for all $\bvarphi\in \bL^r(\Omega)$ and $\psi\in W_0^{1,s}(\Omega)$ there holds
\begin{equation}
  \label{eq:weak-form-main}
  \begin{gathered}
    \ap{\bLambda_{\bu},\bvarphi} = -\ap{\bgrad p,\bvarphi} + \ap{\bff_0,\bvarphi},\\
    \ap{\bgrad\psi,\bu} = - \int_\Omega q\psi + \int_{\Sigma_{\mt{v}}} u_0\psi .
  \end{gathered}
\end{equation}
Our goal is now to show existence for this weak formulation.


% \subsection{Multivalued setting}
% \label{sec:multiv-setting}

% As argued previously, the law operator $\bLambda$ is from this point allowed to be multivalued, so that the velocity-pressure law in \eqref{eq:relation-u-p} actually reads
% \begin{equation}
%   \label{eq:multiv-law}
%   -\bgrad p + f \in \bLambda(\bu).
% \end{equation}
% We are thus allowed to take the following set of convex combinations between $\bLambda_1$ and $\bLambda_2$ as our interface law operator, as suggested by the energetic consideration of Section \ref{sec:energetic-cons}:
% \begin{equation*}
%   \bLambda_\Gamma(\bu) = \left\{ (1 - \tau) \bLambda_1(\bu) + \tau\bLambda_2(\bu) \right\}_{\tau\in L^\infty(\Omega;[0,1])}.
% \end{equation*}
% In other terms, our law operator $\bLambda$ satisfies
% \begin{equation}
%   \label{eq:multiv-heaviside-law}
%   \bLambda(\bu) = (1 - \frakH(\abs{\bu}^2)) \bLambda_1(\bu) + \frakH(\abs{\bu}^2) \bLambda_2(\bu) = \bLambda_1(\bu) + \frakH(\abs{\bu}^2) (\bLambda_2(\bu) - \bLambda_1(\bu)),
% \end{equation}
% where $\frakH \: \R \to 2^{L^\infty(\Omega;[0,1])}$ is given in \eqref{eq:heaviside-multiv}. Our problem thus summarizes as: find a pair $(\bu,p)$ of functions such that
% \begin{equation}
%   \label{eq:main}
%   \begin{gathered}
%     \dive \bu = q \quad \text{on $\Omega$},\\
%     -\bgrad p + \bff \in \bLambda(\bu) \quad \text{on $\Omega$},\\
%     \bu \cdot \bn = b \quad \text{on $\p\Omega$},
%   \end{gathered}
% \end{equation}
% where the law operator $\bLambda$ is of the form \eqref{eq:multiv-heaviside-law}. For any $\tau\in L^\infty(\Omega;[0,1])$ we shall denote by $\frakH_\tau\:\R\to L^\infty(\Omega;[0,1])$ the function defined for all $a\in\R$ by
% \begin{equation*}
%   \frakH_\tau(a) = 
%   \begin{cases}
%     0 & \text{if $a < 1$},\\
%     \tau & \text{if $a = 1$},\\
%     1 & \text{if $a > 1$},
%   \end{cases}
% \end{equation*}
% and 
% \begin{equation*}
%   \bLambda(\tau;\bu) = (1 - \frakH_\tau(\abs{\bu}^2)) \bLambda_1(\bu) + \frakH_\tau(\abs{\bu}^2) \bLambda_2(\bu) = \bLambda_1(\bu) + \frakH_\tau(\abs{\bu}^2) (\bLambda_2(\bu) - \bLambda_1(\bu)).
% \end{equation*}
% With this, our problem amounts to: find a triplet $(\bu,p,\tau)$ with $\tau\in L^\infty(\Omega;[0,1])$ such that 
% \begin{equation}
%   \label{eq:main-tau}
%   \begin{gathered}
%     \dive \bu = q \quad \text{on $\Omega$},\\
%     -\bgrad p + \bff = \bLambda(\tau;\bu) \quad \text{on $\Omega$},\\
%     \bu \cdot \bn = b \quad \text{on $\p\Omega$}.
%   \end{gathered}
% \end{equation}


\section{Existence}
\label{sec:existence}

We state and prove here our results on existence for Problem \eqref{eq:weak-form-main}. We will see that our results depend on the sign of the difference $\lambda_2 - \lambda_1$, where we use the notation
\begin{equation}
  \label{eq:lambdas}
  \lambda_1 := \phi_1(1) \quad \text{and} \quad \lambda_2 := \phi_2(1).
\end{equation}
The strategy is the following: 
\begin{enumerate}
  \item we simplify Problem \eqref{eq:weak-form} on the velocity and pressure fields into an equivalent problem on the velocity field only (cf. \eqref{eq:weak-form-V0});
  \item we derive an energetic formulation whose minimizers are solutions to this simplified problem on the velocity field (cf. \eqref{eq:minimization});
  \item we study the existence of minimizers for this energetic formulation distinguishing the convex case $\lambda_1\leq\lambda_2$ from the nonconvex case $\lambda_1 > \lambda_2$ (cf. Theorems \ref{thm:wp-1-less-than-2} and \ref{thm:wp-1-greater-than-2}).
\end{enumerate}


\subsection{Simplification to a problem on the velocity field}
\label{sec:restriction-V0}

Define the maps $B \: \bL^r(\Omega) \to (W_0^{1,s}(\Omega))^*$ and $\bB^* \: W_0^{1,s}(\Omega) \to (\bL^r(\Omega))^*$  by
\begin{equation}
  \label{eq:B}
  B(\bvarphi)(\psi) = \bB^*(\psi)(\bvarphi) = \ap{\bgrad \psi, \bvarphi} \quad \text{for all $\bvarphi \in \bL^r(\Omega)$ and $\psi\in W_0^{1,s}(\Omega)$},
\end{equation}
Let us introduce the set
\begin{equation*}
  V = \{ \bvarphi \in \bL^r(\Omega) \st \forall\, \psi\in W_0^{1,s}(\Omega),\, \ap{\bgrad \psi,\bvarphi} = 0 \},
\end{equation*}
which satisfies $V = \mathrm{Ker}(B)$. We write $V^\perp\subset \bL^s(\Omega)$ the polar subspace of $V$, that is, $V^\perp = \{ \bg \in \bL^s(\Omega) \st \forall\, \bvarphi\in V,\, \ap{\bg,\bvarphi} = 0\}$, and $\bL^r(\Omega)/V \subset \bL^r(\Omega)$ the quotient space of $\bL^r(\Omega)$ by $V$.

\begin{lem}
  \label{lem:isomorphisms}
  The maps $B$ and $B^*$ in \eqref{eq:B} are isomorphisms from $\bL^r(\Omega)/V$ to $(W_0^{1,s}(\Omega))^*$ and from $W_0^{1,s}(\Omega)$ to $V^\perp$, respectively.
\end{lem}
\begin{proof}
  By Lemma \ref{lem:inf-sup} in the appendix, it suffices to show that there exists $\beta > 0$ such that
    \begin{equation*}
    \inf_{\substack{\psi \in W_0^{1,s}(\Omega)\\ \psi\neq 0}} \sup_{\substack{\bvarphi\in \bL^r(\Omega)\\ \bvarphi\neq \bnull}} \frac{\ap{\bgrad\psi,\bvarphi}}{\norm{\psi}_{W_0^{1,s}(\Omega)}\norm{\bvarphi}_{\bL^r(\Omega)}} \geq \beta.
  \end{equation*}
  To this end, let $\psi\in W_0^{1,s}(\Omega)$ with $\psi \neq 0$. Then we know that
  \begin{equation*}
    \norm{\psi}_{W_0^{1,s}(\Omega)} = \norm{\bgrad\psi}_{\bL^s(\Omega)} = \sup_{\substack{\bvarphi\in \bL^r(\Omega)\\\bvarphi\neq\bnull}} \frac{\ap{\bgrad\psi,\bvarphi}}{\norm{\bvarphi}_{\bL^r(\Omega)}},
  \end{equation*}
  so that
  \begin{equation*}
    1 = \frac{\norm{\psi}_{W_0^{1,s}(\Omega)}}{\norm{\psi}_{W_0^{1,s}(\Omega)}} = \sup_{\substack{\bvarphi\in \bL^r(\Omega)\\\bvarphi\neq\bnull}} \frac{\ap{\bgrad\psi,\bvarphi}}{\norm{\psi}_{W_0^{1,s}(\Omega)}\norm{\bvarphi}_{\bL^r(\Omega)}}.
  \end{equation*}
  Taking above the infimum over all $\psi \in W_0^{1,s}(\Omega)$ with $\psi\neq 0$ ends the proof.
\end{proof}

Now, via the following two lemmas, we simplify our weak formulation \eqref{eq:weak-form-main} into a problem restricted to $V$ (cf. \eqref{eq:weak-form-V0} below). 
\begin{lem}
  \label{lem:bdry-V0}
  There exists a unique $\hat\bu\in \bL^r(\Omega)/V$ such that
  \begin{equation*}
    \ap{\bgrad \psi,\hat\bu} = -\int_\Omega q\psi + \int_{\Sigma_{\mt{v}}} u_0\psi \quad \text{for all $\psi\in W_0^{1,s}(\Omega)$}.
  \end{equation*}
\end{lem}
\begin{proof}
  For all $\psi\in W_0^{1,s}(\Omega)$, let
  \begin{equation*}
    F(\psi) = -\int_\Omega q\psi + \int_{\Sigma_{\mt{v}}} u_0\psi. 
  \end{equation*}
  Since we are assuming that $q\in L^r(\Omega)$ and $u_0\in W^{1,r}(\Omega)$ (and so the trace $u_0\in L^r(\p\Omega)$), the map $F$ is a well-defined linear map from $W_0^{1,s}(\Omega)$ into $\R$, i.e., $F\in (W_0^{1,s}(\Omega))^*$. By Lemma \ref{lem:isomorphisms}, we thus know there exists a unique $\hat\bu \in \bL^r(\Omega)/V$ such that
  \begin{equation*}
    \ap{\bgrad\psi,\hat\bu} = B(\hat\bu)(\psi) = F(\psi) = -\int_\Omega q\psi + \int_{\Sigma_{\mt{v}}} u_0\psi \quad \text{for all $\psi\in W_0^{1,s}(\Omega)$}, 
  \end{equation*}
  which is the desired result.
\end{proof}
\begin{lem}
  The weak formulation \eqref{eq:weak-form-main} is equivalent to the following problem: find $\bv\in V$ such that there exists $\bLambda_{\bv} \in \bLambda(\bv+\hat\bu)$ satisfying
  \begin{equation}
    \label{eq:weak-form-V0}
    \ap{\bLambda_{\bv},\bvarphi} = \ap{\bff_0,\bvarphi} \quad \text{for all $\bvarphi \in V$},
  \end{equation}
  where $\hat\bu$ is given by Lemma \ref{lem:bdry-V0}.
\end{lem}
\begin{proof}
  We first suppose that $(\bu,p)$ is solution to Problem \eqref{eq:weak-form-main}. Then we decompose $\bu$ as $\bu = (\bu - \hat\bu) + \hat\bu =: \bv + \hat\bu$. By \eqref{eq:weak-form-main}, there exists $\bLambda_{\bv} \in \bLambda(\bu) = \bLambda(\bv+\hat\bu)$ such that
  \begin{equation*}
    \ap{\bLambda_{\bv},\bvarphi} = \ap{\bff_0,\bvarphi} \quad \text{for all $\bvarphi \in V$}.
  \end{equation*}
Furthermore, for all $\psi\in W_0^{1,s}(\Omega)$ we find $\ap{\bgrad\psi,\bv} = \ap{\bgrad\psi,\bu} - \ap{\bgrad\psi,\hat\bu} = 0$, so that $\bv\in V$ and $\bv$ satisfies Problem \eqref{eq:weak-form-V0}.

  Suppose now that $\bv$ satisfies Problem \eqref{eq:weak-form-V0}. Then, $\bLambda_{\bv} - \bff_0 \in V^{\mathrm{\perp}}$. By Lemma \ref{lem:isomorphisms} we know $\bB^*$ is an isomorphism from $W_0^{1,s}(\Omega)$ to $V^{\mathrm{\perp}}$, so that there exists a unique $p\in W_0^{1,s}(\Omega)$ with
  \begin{equation*}
    \ap{\bLambda_{\bv} - \bff_0,\bvarphi} = \bB^*(-p)(\bvarphi) = -\ap{\bgrad p,\bvarphi} \quad \text{for all $\bvarphi\in\bL^r(\Omega)$}.
  \end{equation*}
Then, writing $\bu = \bv + \hat\bu$ we get
\begin{equation*}
  \ap{\bgrad\psi,\bu} = \ap{\bgrad\psi,\bv} + \ap{\bgrad\psi,\hat\bu} = \ap{\bgrad\psi,\hat\bu}  = - \int_\Omega q\psi + \int_{\Sigma_{\mt{v}}} u_0\psi,
\end{equation*}
since $\bv\in V$. We thus have that $(\bu,p)$ satisfies Problem \eqref{eq:weak-form-main}, with $p$ unique.
\end{proof}

\subsection{Energetic formulation}
\label{sec:energ-form}

% In the following we write $\bLambda_0\:V \to (V)^*$ the operator given by
% \begin{equation*}
%   \bLambda_0(\bv) = \bLambda(\bv + \hat\bu) \quad \text{for all $\bv\in V$},
% \end{equation*}
% where $\hat\bu$ is defined as in Lemma \ref{lem:bdry-V0}. 

We first recall the definition of Fréchet subdifferential and strong local minimizer in our setting:
\begin{defn}[Fréchet subdifferential and strong local minimizer]
  Let $\F\:V\to \R$. For all $\bv\in V$ we define the \emph{(Fréchet) subdifferential} $\p\F(\bv)$ of $\F$ at $\bv$ by:
  \begin{equation*}
    \bg_{\bv} \in \p\F(\bv) \iff \bg_{\bv} \in V^*\; \text{ and }\; \forall\, \bvarphi\in V,\; \liminf_{\delta\to 0^+} \frac{\F(\bv+\delta\bvarphi) - \F(\bv)}{\delta} \geq \ap{\bg_{\bv},\bvarphi}.
  \end{equation*}
  We say that $\bv\in V$ is a \emph{(strong) local minimizer} of $\F$ if for all $\bvarphi\in V$ there exists $\eta>0$ such that $\F(\bv +\delta\bvarphi) \geq \F(\bv)$ for all $\delta\in[0,\eta)$.
\end{defn}

\begin{rem}
  \label{rem:minimizers}
  The important property of the subdifferential to keep in mind here is that $\bv\in V$ is a local minimizer of a functional $\F\:V\to \R$ if and only if there exists $\bg_{\bv}\in \p\F(\bv)$ such that $\ap{\bg_{\bv},\bvarphi} = 0$ for all $\bvarphi\in V$.   
\end{rem}

We write $\Psi\:[0,\infty)\to \R$ the function given by
\begin{equation}
  \label{eq:psi}
  \Psi(a) = \begin{cases} \Phi_1(a) & \text{for all $a\leq 1$},\\ \Phi_2(a) & \text{for all $a> 1$}, \end{cases}
\end{equation}
where $\Phi_1,\Phi_2\:[0,\infty) \to \R$ are primitives of $\tfrac{\phi_1}{2}$ and $\tfrac{\phi_2}{2}$ (cf. \eqref{eq:law-form}) such that $\Phi_1(1) = \Phi_2(1) = 0$. We define the \emph{dissipation} $\D\:V \to \R$ by
\begin{equation}
  \label{eq:dissipation}
  \D(\bv) = \int_\Omega \Psi(\norm{\bv + \hat\bu}^2) \quad \text{for all $\bv\in V$}.
\end{equation}
Thanks to our assumptions on $\phi_1$ and $\phi_2$ we easily get that the domain of $\D$ is indeed all of $V$, and it is thus a well-defined functional from $V$ into $\R$. Consider the following problem: find $\bv\in V$ such that there exists $\bg_{\bv}\in \p\D(\bv)$ satisfying
\begin{equation}
  \label{eq:energy-form-V0}
  \ap{\bg_{\bv},\bvarphi} = \ap{\bff_0,\bvarphi} \quad \text{for all $\bvarphi\in V$}.
\end{equation}
The following result holds:
\begin{lem}
  \label{lem:energy-implies-sol}
  Any solution to Problem \eqref{eq:energy-form-V0} is also solution to Problem \eqref{eq:weak-form-V0}.
\end{lem}
\begin{proof}
  Suppose that $\bv\in V$ is solution to Problem \eqref{eq:energy-form-V0}. Then we can pick $\bg_{\bv}\in\p\D(\bv)\subset\bL^s(\Omega)$ so that \eqref{eq:energy-form-V0} holds. By definition, for all $\bvarphi\in V$ we must have
  \begin{equation*}
    \liminf_{\delta\to0^+} \frac{\D(\bv+\delta\bvarphi) - \D(\bv)}{\delta} \geq \ap{\bg_{\bv},\bvarphi}.
  \end{equation*}
    Write $V_1$ the subset of $V$ consisting of the functions which are supported in $\Omega_1(\bv+\hat\bu)$. Then, for all $\bvarphi\in V_1$, we get
  \begin{equation*}
    \liminf_{\delta\to0^+} \frac{1}{\delta} \int_{\Omega_1(\bv+\hat\bu)} \left( \Psi(\norm{\bv +\delta\bvarphi + \hat\bu}^2) - \Phi_1(\norm{\bv + \hat\bu}^2) \right) \geq \ap{\bg_{\bv},\bvarphi}
  \end{equation*}
  and
  \begin{equation*}
    \liminf_{\delta\to0^+} \frac{1}{\delta} \int_{\Omega_1(\bv+\hat\bu)} \left( \Psi(\norm{\bv -\delta\bvarphi + \hat\bu}^2) - \Phi_1(\norm{\bv + \hat\bu}^2) \right) \geq -\ap{\bg_{\bv},\bvarphi},
  \end{equation*}
  which, by Lebesgue's dominated convergence theorem and the differentiability of $\Phi_1$, yield
  \begin{equation*}
    \int_\Omega \bLambda_1(\bv+\hat\bu)\cdot\bw = \int_{\Omega_1(\bv+\hat\bu)} \phi_1(\norm{\bv+\hat\bu}^2) (\bv +\hat\bu)\cdot\bvarphi  \geq \ap{\bg_{\bv},\bvarphi}
  \end{equation*}
  and
  \begin{equation*}
    -\int_\Omega \bLambda_1(\bv+\hat\bu)\cdot\bw = -\int_{\Omega_1(\bv+\hat\bu)} \phi_1(\norm{\bv+\hat\bu}^2) (\bv +\hat\bu)\cdot\bw  \geq -\ap{\bg_{\bv},\bvarphi}.
  \end{equation*}
  All in all we get
  \begin{equation*}
    \ap{\bg_{\bv},\bvarphi} = \ap{\bLambda_1(\bv+\hat\bu),\bvarphi} \quad \text{for all $\bvarphi\in V_1$}.
  \end{equation*}
  Similarly, denoting by $V_2$ the subset of $V$ consisting of the functions which are supported in $\Omega_2(\bv+\hat\bu)$, we get
  \begin{equation*}
    \ap{\bg_{\bv},\bvarphi} = \ap{\bLambda_2(\bv+\hat\bu),\bvarphi} \quad \text{for all $\bvarphi\in V_2$}.
  \end{equation*}
  Thus, the function defined by
  \begin{equation*}
    \bLambda_{\bv} =
    \begin{cases}
      \bLambda_1(\bv+\hat\bu) & \text{on $\Omega_1(\bv+\hat\bu)$},\\
      \bg_{\bv} & \text{on $\Gamma(\bv+\hat\bu)$},\\
      \bLambda_2(\bv+\hat\bu) & \text{on $\Omega_2(\bv+\hat\bu)$},\\
    \end{cases}
  \end{equation*}
  is such that $\ap{\bLambda_{\bv},\bvarphi} = \ap{\bg_{\bv},\bvarphi}$ for all $\bvarphi\in V$. Therefore, from \eqref{eq:energy-form-V0} we obtain
  \begin{equation*}
    \ap{\bLambda_{\bv},\bvarphi} = \ap{\bff_0,\bvarphi} \quad \text{for all $\bvarphi\in V$}.
  \end{equation*}
  Moreover $\bLambda_{\bv}\in\bLambda(\bv+\hat\bu)$, where we recall that $\bLambda$ is as in \eqref{eq:law-combined}. Hence $\bv$ is a solution to Problem \eqref{eq:weak-form-V0}.
  % For all $\bw \in V$ and $\delta>0$ we note that
  % \begin{align*}
  %   \D(\bv+\delta\bw) - \D(\bv) &= \int_\Omega \left( \Psi(\abs{\bv +\delta\bw + \hat\bu}^2) - \Psi(\abs{\bv + \hat\bu}^2) \right)\\
  %   &= \int_{\Omega_1(\bv+\hat\bu)} \left( \Psi(\abs{\bv +\delta\bw + \hat\bu}^2) - \Phi_1(\abs{\bv + \hat\bu}^2) \right)\\
  %   &\quad + \int_{\Omega_2(\bv+\hat\bu)} \left( \Psi(\abs{\bv +\delta\bw + \hat\bu}^2) - \Phi_2(\abs{\bv + \hat\bu}^2) \right)\\
  %   &\quad + \int_{\Gamma(\bv+\hat\bu)} \Psi(\abs{\bv +\delta\bw + \hat\bu}^2).
  % \end{align*}
\end{proof}

We now define the \emph{energy} $\E\:V \to \R$ associated to $\D$ by 
\begin{equation*}
  \E(\bv) = \D(\bv) - \ap{\bff_0,\bv} \quad \text{for all $\bv\in V$}.
\end{equation*}
Let us write $M_\E\subset V$ the set of local minimizers of $\E$. Note that we may have $M_\E=\emptyset$. Thanks to Remark \ref{rem:minimizers}, Problem \eqref{eq:energy-form-V0} is in turn equivalent to the following minimization problem: find $\bv\in V$ such that 
\begin{equation}
  \label{eq:minimization}
  \bv \in M_\E.
\end{equation}
By Lemma \ref{lem:energy-implies-sol} it therefore suffices to find a solution to Problem \eqref{eq:minimization} in order to get the desired existence result on Problem \eqref{eq:weak-form-main}. The rest of this section will thus be solely dedicated to solving Problem \eqref{eq:minimization}.


\subsection{Case $\lambda_1\leq\lambda_2$}
\label{sec:case-1-less-than-2}

The result we wish to show here is the following:
\begin{thm}[Existence and uniqueness when $\lambda_1 \leq \lambda_2$]
  \label{thm:wp-1-less-than-2}
  Suppose that $\lambda_1 \leq \lambda_2$. Then, Problem \eqref{eq:minimization} has a unique solution.
\end{thm}
\begin{proof}
  Let us prove that the integrand $\Psi\circ\norm{\cdot}^2$ (cf. \eqref{eq:psi}) of $\D$ is strictly convex. Define the functions $\bar\Phi_1,\bar\Phi_2\:[0,\infty)\to\R$ by
  \begin{equation*}
    \bar \Phi_1(a) = 
    \begin{cases}
      \Phi_1(a) & \text{for all $a\leq1$},\\
      \lambda_1(a-1) & \text{for all $a> 1$},
    \end{cases}
    \quad \text{and} \quad 
    \bar \Phi_2(a) = 
    \begin{cases}
      \lambda_2(a-1) & \text{for all $a\leq1$},\\
      \Phi_2(a) & \text{for all $a> 1$}.\\
    \end{cases}
  \end{equation*}
  Then $\bar\Phi_1$ and $\bar\Phi_2$ are differentiable with 
  \begin{equation*}
    \bar \Phi_1'(a) = 
    \begin{cases}
      \phi_1(a) & \text{for all $a\leq1$},\\
      \lambda_1 & \text{for all $a> 1$},
    \end{cases}
    \quad \text{and} \quad 
    \bar \Phi_2'(a) = 
    \begin{cases}
      \lambda_2 & \text{for all $a\leq1$},\\
      \phi_2(a) & \text{for all $a> 1$}.\\
    \end{cases}
  \end{equation*}
  Since $\phi_1$ and $\phi_2$ are increasing and $\phi_1(1) = \lambda_1$ and $\phi_2(1) = \lambda_2$, the derivatives $\bar\Phi_1'$ and $\bar\Phi_2'$ are also increasing so that $\bar\Phi_1$ and $\bar\Phi_2$ are convex. Furthermore, because $\lambda_1\leq \lambda_2$ and $\phi_2$ is decreasing, we have $\bar\Phi_2'(a) \geq \bar\Phi_1'(a)$ for all $a>1$; thus, the fact that $\Phi_1(1) = \Phi_2(1)$ yields $\bar\Phi_1(a)\leq \bar\Phi_2(a)$ for all $a>1$. Similarly, we get that $\bar\Phi_1(a)\geq \bar\Phi_2(a)$ for all $a<1$. Let $a,b \in [0,\infty)$ and $t\in[0,1]$. If $a,b \leq 1$, then $(1-t)a+tb\leq1$ and
  \begin{align*}
    \Psi((1-t) a + tb) &= \Phi_1((1-t) a + tb) = \bar\Phi_1((1-t) a + tb)\\
    &\leq (1-t)\bar\Phi_1(a) + t\bar\Phi_1(b) = (1-t)\Psi(a) + t\Psi(b),
  \end{align*}
  and similarly if $a,b > 1$. If now $a\leq1$, $b>1$ and $(1-t)a+tb\leq1$, then we have
  \begin{align*}
    \Psi((1-t) a + tb) &= \Phi_1((1-t) a + tb) = \bar\Phi_1((1-t) a + tb)\\
    &\leq (1-t)\bar\Phi_1(a) + t\bar\Phi_1(b) \leq (1-t)\bar\Phi_1(a) + t\bar\Phi_2(b) = (1-t)\Psi(a) + t\Psi(b),
  \end{align*}
  and similarly if $(1-t)a+tb>1$ or $a>1$ and $b\leq1$. In all cases, we see that
  \begin{equation*}
    \Psi((1-t)a+tb) \leq (1-t)\Psi(a) + t\Psi(b),
  \end{equation*}
  so that $\Psi$ is convex. Since $\phi_1$ and $\phi_2$ are increasing we get that $\Psi$ is also increasing. Therefore, the function $\Psi\circ\norm{\cdot}^2$ is strictly convex.  

  We now want to use the direct method of the calculus of variations to show that $\E$ has in fact a unique global (and thus local) minimizer. Let $(\bv_n)_{n\in\N} \subset V$ be a minimizing sequence for $\E$. Then we know there exists $N\in\N$ large enough and $K > 0$ such that $\E(\bv_n) < K$ for all $n>N$. Without loss of generality we can therefore assume that the sequence $(\E(\bv_n))_{n\in\N}$ is bounded by some constant $K>0$. Hence, thanks to the left-hand inequality in \eqref{eq:bound-phi2}, for all $n\in\N$ we have
  \begin{align*}
    K > \E(\bv_n) &= \int_{\Omega_1(\bv_n+\hat\bu)} \Phi_1(\norm{\bv_n+\hat\bu}^2) + \int_{\Omega_2(\bv_n+\hat\bu)} \Phi_2(\norm{\bv_n+\hat\bu}^2)- \int_\Omega \bff_0\cdot\bv_n\\
              &\geq \Phi_1(0) \norm{\Omega} + c\int_{\Omega_2(\bv_n+\hat\bu)} \norm{\bv_n+\hat\bu}^r - \norm{\bff_0}_{\bL^s(\Omega)}^s\norm{\bv_n+\hat\bu}_{\bL^r(\Omega)}^r\\
              &\geq (\Phi_1(0)-c) \abs{\Omega} + c\norm{\bv_n+\hat\bu}_{\bL^r(\Omega)}^r - \norm{\bff_0}_{\bL^s(\Omega)}\norm{\bv_n+\hat\bu}_{\bL^r(\Omega)},
  \end{align*}
which shows that the sequence $(\norm{\bv_n}_{\bL^r(\Omega)})_{n\in\N}$ is bounded. Thus we can extract a subsequence from $(\bv_n)_{n\in\N}$, still denoted $(\bv_n)_{n\in\N}$ which converges weakly to some $\bv\in\bL^r(\Omega)$. Since further $V$ is weakly closed we in fact have $\bv\in V$. Because $\Psi\circ\norm{\cdot}^2$ is convex, the energy $\E$ is weakly lower semicontinuous. We therefore yield
\begin{equation*}
  \inf_{\bw\in V}\E(\bw) = \liminf_{n\to\infty} \E(\bv_n) \geq \E(\bv) \geq \inf_{\bw\in V}\E(\bw),
\end{equation*}
so that $\E(\bv) = \inf_{\bw\in V}\E(\bw)$ and $\bv$ is a global minimizer of $\E$ and so $\bv\in M_\E$.

To show that $M_\E$ is a singleton it is enough to prove that $\E$ is strictly convex. Let $\bv,\bw\in V$ and $t\in(0,1)$. Suppose furthermore that $\bv\neq\bw$ and write $A\subset\Omega$ the set where $\bv$ and $\bw$ are different; the Lebesgue measure of $A$ is therefore positive. Using the strict convexity of $\Psi\circ\norm{\cdot}^2$ we get
  \begin{align*}
    \D((1-t)\bv+t\bw) &= \int_\Omega\Psi(\norm{(1-t)\bv+t\bw+\hat\bu}^2) = \int_\Omega \Psi(\norm{(1-t)(\bv+\hat\bu)+t(\bw+\hat\bu)}^2)\\
                      &= (1-t)\int_{\Omega\setminus A} \Psi(\norm{\bv+\hat\bu}^2) + t\int_{\Omega\setminus A} \Psi(\norm{\bw+\hat\bu}^2)\\
                      &\quad + \int_{A} \Psi(\norm{(1-t)(\bv+\hat\bu)+t(\bw+\hat\bu)}^2)\\
                      &< (1-t)\int_{\Omega\setminus A} \Psi(\norm{\bv+\hat\bu}^2) + t\int_{\Omega\setminus A} \Psi(\norm{\bw+\hat\bu}^2)\\
                      &\quad + \int_{A} \Psi((1-t)\norm{\bv+\hat\bu}^2 + t\norm{\bw+\hat\bu}^2)\\
                      &\leq (1-t)\int_{\Omega\setminus A} \Psi(\norm{\bv+\hat\bu}^2) + t\int_{\Omega\setminus A} \Psi(\norm{\bw+\hat\bu}^2)\\
                      &\quad + (1-t)\int_{A} \Psi(\norm{\bv+\hat\bu}^2) +t\int_{A} \Psi(\norm{\bw+\hat\bu}^2)\\
                      &= (1-t)\int_\Omega \Psi(\norm{\bv+\hat\bu}^2) +t\int_\Omega \Psi(\norm{\bw+\hat\bu}^2) = (1-t)\D(\bv) + t\D(\bw),
  \end{align*}
  so that the dissipation $\D$ is strictly convex. Consequently, the energy $\E$ is also strictly convex and the proof is over. 
\end{proof}



\subsection{Case $\lambda_1 > \lambda_2$}
\label{sec:case-2-less-than-1}

This case is more difficult to tackle than the case $\lambda_1 \leq \lambda_2$. Indeed, we lose the convexity of the integrand $\Psi\circ\norm{\cdot}^2$ (cf. proof of Theorem \ref{thm:wp-1-less-than-2}), which by Tonelli's theorem of functional analysis means that $\E$ is not weakly lower semicontinuous. As a consequence we cannot use the direct method of the calculus of variations to deduce the existence of a minimizer to $\E$. 

To simplify our task at this point, we shall restrict to the one-dimensional case (i.e., $d=1$) and leave the higher-dimensional case for future investigation. The results we present here therefore apply to the numerical experiments we present below. The one-dimensional case is simpler since we can easily characterize the space $\bV =: V$ depending on the boundary conditions, as will be clear from the proof of the following theorem:
\begin{thm}[Existence and uniqueness when $\lambda_1 > \lambda_2$]
  \label{thm:wp-1-less-than-2}
  Suppose that $\lambda_1 > \lambda_2$ and $d=1$. If $\mt{Vol}^0(\Sigma_{\mt{v}}) = 0$, then Problem \eqref{eq:minimization} has a solution. If instead $\mt{Vol}^0(\Sigma_{\mt{v}}) > 0$, then Problem \eqref{eq:minimization} has a unique solution.
\end{thm}
\begin{proof}
Without loss of generality, take $\Omega = [0,1]$. 

Suppose first that $\mt{Vol}^0(\Sigma_{\mt{v}}) = 0$. Let us characterize the space $V$ in this case. To this end, note that any $\eta\in V$ such that $\int_0^1 \eta = 0$ has a primitive in $W_0^{1,s}(\Omega)$; indeed, the function $\psi\: \Omega \to \R$ defined by
\begin{equation*}
    \psi(x) = \int_0^x \eta \quad \text{for all $x\in(0,1)$}  
\end{equation*}
satisfies $\psi' = \eta$ and $\psi(0) = \psi(1) = 0$. Let now $v \in V$ and define $\eta\in V$ as
\begin{equation*}
    \eta(x) = v(x) - \int_0^1 v  \quad \text{for all $x\in(0,1)$},
\end{equation*}
so that obviously $\int_0^1 \eta = 0$. Compute, for all $v\in V$,
\begin{align*}
    \int_0^1 \varphi v &= \int_0^1 \varphi \left( v - \int_0^1 v \right) + \int_0^1 v \int_0^1 v\\
    &= \int_0^1 \varphi \eta + \int_0^1 \varphi \int_0^1 v\\
    &= \int_0^1 \varphi \psi' + \int_0^1 \varphi \int_0^1 v\\
    &= \int_0^1 \varphi \int_0^1 v,
\end{align*}
so that
\begin{equation*}
    \int_0^1 v \left( v - \int_0^1 v \right) = 0
\end{equation*}
and therefore $v = \int_0^1 v$. Hence the space $V$ is the set of constant functions on $[0,1]$ and we can identify $V$ with $\R$. \comment{Possiamo quindi minimizzare l'energia $E$ sullo spazio $\R$... Non è convessa quindi non abbiamo l'unicità, ma l'esistenza c'è.}

Suppose now that $\mt{Vol}^0(\Sigma_{\mt{v}}) > 0$. \comment{In questo caso ancora più semplice: $V = \{0\}$}
\end{proof}


%Instead we define a convex problem associated to \eqref{eq:minimization} and show that whenever minimizers of this associated problem satisfy some bounds, they coincide with minimizers of the original nonconvex problem. 

%\comment{Idea:

%Our strategy is the following. We define a secondary minimization problem on the functional $\hat \E_0$ defined by
%\begin{equation*}
%  \hat \E_0(\bv) = \int_\Omega \hat\Psi(\abs{\bv+\hat\bu}^2) - \ap{\bff,\bv},
%\end{equation*}
%where $\hat \Psi$ is the convex envelope of $\Psi$. (This should correspond to the double convex conjugate of $\Psi$.) Then $\hat\Psi \leq \Psi$ and $\hat \Psi$ is differentiable and convex. Because $\Psi$ is piecewise convex on the intervals $[0,1]$ and $[1,\infty)$ we actually have values $\hat \lambda_1 < 1$ and $\hat \lambda_2 > 1$ such that
%\begin{equation*}
%  \hat\Psi(a) = \Psi(a) \quad \text{for all $a<\hat\lambda_1$ and $a>\hat\lambda_2$}.
%\end{equation*}
%$\hat\E_0$ has a unique minimizer $\hat\bv$. We have the following result:
%\begin{thm}[Existence and uniqueness when $\lambda_1 > \lambda_2$]
%  Suppose that $\lambda_1 > \lambda_2$. Suppose that $\hat\bv$ satisfies the following condition:
%  \begin{equation*}
%    \abs{\hat \bv(x)} \not\in [\hat\lambda_1,\hat \lambda_2] \quad \text{for almost every $\bx\in\Omega$}.
%  \end{equation*}
%Then, Problem \eqref{eq:weak-form-V0} has a unique solution.
%\end{thm}
%\begin{proof}
%  We have in this case, for all $\bv\in V$,
%  \begin{equation*}
%    \E_0(\hat\bv) = \hat\E_0(\hat\bv) \leq \hat \E_0(\bv) \leq \E_0(\bv).
%  \end{equation*}
%  Thus $\hat\bv$ is a minimizer of $\E_0$. Because a convex analysis theorem tells us that $\inf \hat\E_0 = \inf \E_0$, this must be the unique minimizer of $\E_0$ (check...).
%\end{proof}
%
%In the Darcy-Darcy case, this condition on $\hat \bv$ should hold when $\bff\in V^\perp$.
%}


\comment{Questions for later (with student?):
  \begin{itemize}
    \item Which law in $\p \D$ is being picked at the interface?
    \item Compute $\p\D$ on the interface.
    \item What is the dimension of the interface?
    \item Existence result when $\lambda_1 > \lambda_2$ and $d>1$.    
    \item Extend the result to tensor permeabilities.
    \item Can we add $p$ in the law operator?
  \end{itemize}
}


% The proof of this theorem will be based on the multivalued version of the Minty--Browder theorem \comment{referenza}, which we recall reads as follows:
% \begin{thm}[Minty--Browder]
%   Let $X$ be a reflexive Banach space with dual $X^*$. Let $T_1\: X \to X^*$ be a single-valued, bounded, coercive, hemicontinuous, monotone operator with $\dom(T_1) = X$. Let furthermore $T_2 \: X \to 2^{X^*}$ be a multivalued maximal monotone operator with $\dom(T_2) = X$. Then, the image of the multivalued operator $T_1 + T_2$ is all of $X^*$, i.e., for all $y\in X^*$ there exists $x\in X$ such that $y\in T(x)$.
% \end{thm}

% Note first that because $V$ is closed and $\bL^r(\Omega)$ is reflexive, $V$ is also reflexive. Recalling \eqref{eq:multiv-heaviside-law} we see that our law on $V$ can be written 
% \begin{equation*}
%   \bLambda_0 = \bLambda_{0,1} + \bLambda_{0,21},
% \end{equation*}
% where $\bLambda_{0,21} \: V \to (V)^*$ is the multivalued operator defined by
% \begin{equation*}
%   \bLambda_{0,21}(\bv) = \frakH(\abs{\bv + \hat\bu}^2)(\bLambda_{0,2}(\bv) - \bLambda_{0,1}(\bv)) \quad \text{for all $\bv\in V$}.
% \end{equation*}
% The existence part of Theorem \ref{thm:wp-1-less-than-2} would be a direct consequence of $\bLambda_{0,1}$ being bounded, coercive, hemicontinuous and monotone on the one hand, and $\bLambda_{0,21}$ being maximal on the other hand. We focus on this task in the next two lemmas.

% \begin{lem}
%   The operator $\bLambda_{0,1}$ is bounded, coercive, hemicontinuous and monotone.
% \end{lem}
% \begin{proof}
%   We show in order that $\bLambda_{0,1}$ is bounded, coercive, hemicontinuous and monotone.

%   \medskip
%   \noindent \ul{Boundedness.} We want to show that $\bLambda_{0,1}$ maps bounded sets of $V$ to bounded sets of $(V)^*$. To this end, let $\bv\in V$ be such that $\norm{\bv}_{\bL^r(\Omega)} \leq R$ for some $R>0$. Thanks to \eqref{eq:bound-phi2} and \eqref{eq:bound-phi1}, setting $\bu = \bv + \hat\bu$ and $\sigma = \sup_{a\in[0,1]}\phi_1(a)$ we get
%   \begin{align*}
%     \norm{\bLambda_{0,1}(\bv)}_{\bL^s(\Omega)}^s &= \norm{\phi_1(\abs{\bu}^2)\bu}_{\bL^s(\Omega)}^s = \int_\Omega \abs{\phi_1(\abs{\bu}^2)\bu}^s\\
%     &\leq \sigma^s \int_{\Omega_1(\bu)} \abs{\bu}^s + \int_{\Omega_2(\bu)} \abs{\phi_1(\abs{\bu}^2)\bu}^s + \int_{\Gamma(\bu)} \abs{\phi_1(\abs{\bu}^2)\bu}^s\\
%     &\leq \sigma^s \int_\Omega \abs{\bu}^s + \int_\Omega \abs{\phi_1(\abs{\bu}^2)\bu}^s + \lambda_1^s \abs{\Omega}\\
%     &\leq \sigma^s\norm{\bu}_{\bL^s(\Omega)}^s + 2^{1-s} C^s \left( \int_\Omega \abs{\bu}^{(r-1)s} + \int_\Omega \abs{\bu}^s \right) + \lambda_1^s \abs{\Omega}\\
%     &= \sigma^s\norm{\bu}_{\bL^s(\Omega)}^s + 2^{1-s} C^s\left( \norm{\bu}_{\bL^r(\Omega)}^r + \norm{\bu}_{\bL^s(\Omega)}^s \right) + \lambda_1^s \abs{\Omega}\\
%     &\leq C_\Omega \sigma^s\norm{\bu}_{\bL^r(\Omega)}^s + 2^{1-s} C^s (\norm{\bu}_{\bL^r(\Omega)}^r + C_\Omega \norm{\bu}_{\bL^r(\Omega)}^s) + \lambda_1^s \abs{\Omega}\\
%     &\leq 2^{1-s} C^s (\norm{\bv}_{\bL^r(\Omega)} + \norm{\hat\bu}_{\bL^r(\Omega)})^r + C_\Omega(2^{1-s} C^s + \sigma^s) (\norm{\bv}_{\bL^r(\Omega)}+ \norm{\hat\bu}_{\bL^r(\Omega)})^s + \lambda_1^s \abs{\Omega}\\
%     &\leq 2^{1-s} C^s (R + \norm{\hat\bu}_{\bL^r(\Omega)})^r + C_\Omega(2^{1-s} C^s + \sigma^s) (R+ \norm{\hat\bu}_{\bL^r(\Omega)})^s + \lambda_1^s \abs{\Omega},
%   \end{align*}
%   where $C_\Omega>0$ is a constant depending on the Lebesgue measure of the bounded set $\Omega$, so that 
%   \begin{equation*}
%     \norm{\bLambda_{0,1}(\bv)}_{\bL^s(\Omega)} \leq (2^{1-s} C^s (R + \norm{\hat\bu}_{\bL^r(\Omega)})^r + C_\Omega(2^{1-s} C^s + \sigma^s) (R+ \norm{\hat\bu}_{\bL^r(\Omega)})^s + \lambda_1^s \abs{\Omega})^{1/s} < \infty.
%   \end{equation*}
%   By arbitrariness of $R$, this yields the boundedness of $\bLambda_{0,1}$.

%   \medskip
%   \noindent \ul{Coercivity.} Let $\bv\in V$. Then, again setting $\bu = \bv + \hat\bu$ and $\sigma = \sup_{a\in[0,1]} \phi_1(a)$, we have
%   \begin{align*}
%     \ap{\bLambda_{0,1}(\bv),\bv} &= \int_\Omega \phi_1(\abs{\bu}^2) \bu\cdot \bv = \int_\Omega \phi_1(\abs{\bu}^2) \bu\cdot \bu - \int_\Omega \phi_1(\abs{\bu}^2) \bu \cdot \hat\bu\\
%     &\geq \int_{\Omega_2(\bu)} \phi_1(\abs{\bu}^2) \abs{\bu}^2 - \int_\Omega \bLambda_{0,1}(\bv) \cdot \hat\bu\\
%     &= \int_{\Omega} \phi_1(\abs{\bu}^2) \abs{\bu}^2 - \int_{\Omega_1(\bu)} \phi_1(\abs{\bu}^2) \abs{\bu}^2 - \int_{\Gamma(\bu)} \phi_1(\abs{\bu}^2) \abs{\bu}^2 - \int_\Omega \bLambda_{0,1}(\bv) \cdot \hat\bu\\
%     &\geq \int_{\Omega} \phi_1(\abs{\bu}^2) \abs{\bu}^2 - (\sigma+\lambda_1) \abs{\Omega} - \norm{\bLambda_{0,1}(\bv)}_{\bL^s(\Omega)}\norm{\hat\bu}_{\bL^r(\Omega)}\\
%     &\geq c\norm{\bu}_{\bL^r(\Omega)}^r - (\sigma+\lambda_1) \abs{\Omega} - \norm{\bLambda_{0,1}(\bv)}_{\bL^s(\Omega)}\norm{\hat\bu}_{\bL^r(\Omega)}.
%   \end{align*}
%   Following the above computation for boundedness, we further get
%   \begin{align*}
%     \ap{\bLambda_{0,1}(\bv),\bv} &\geq c \norm{\bv+\hat\bu}_{\bL^r(\Omega)}^r\\
%     &\quad - (2^{1-s} C^s (R + \norm{\hat\bu}_{\bL^r(\Omega)})^r + C_\Omega(2^{1-s} C^s + \sigma^s) (R+ \norm{\hat\bu}_{\bL^r(\Omega)})^s + \lambda_1^s \abs{\Omega})^{1/s}\norm{\hat\bu}_{\bL^r(\Omega)}\\
%     &\geq c \norm{\bv+\hat\bu}_{\bL^r(\Omega)}^r - P(\norm{\bv}_{\bL^r(\Omega)}),
%   \end{align*}
%   for some $P\:\R \to \R$ such that $P(a)a^{1-r} \to p$ as $a\to\infty$, with $p\in \R$, and so, when $\bv\neq\bnull$,
%    \begin{equation*}
%      \frac{\ap{\bLambda_{0,1}(\bv),\bv}}{\norm{\bv}_{\bL^r(\Omega)}} \geq c \frac{\norm{\bv+\hat\bu}_{\bL^r(\Omega)}^r}{\norm{\bv}_{\bL^r(\Omega)}} - \frac{P(\norm{\bv}_{\bL^r(\Omega)})}{\norm{\bv}_{\bL^r(\Omega)}} = c \norm{\bv}_{\bL^r(\Omega)}^{r-1} + Q(\norm{\bv}_{\bL^r(\Omega)}),
%    \end{equation*}
%    for some $Q\:\R \to \R$ such that $Q(a)a^{2-r}\to q$ as $a\to\infty$, with $q\in\R$. We therefore get
%    \begin{equation*}
%      \frac{\ap{\bLambda_{0,1}(\bv),\bv}}{\norm{\bv}_{\bL^r(\Omega)}} \to \infty \quad \text{as $\norm{\bv}_{\bL^r(\Omega)} \to \infty$},
%    \end{equation*}
%    which shows coercivity of $\bLambda_{0,1}$.

%    \medskip
%    \noindent \ul{Hemicontinuity.} Let $\bv,\bw,\bvarphi\in V$. Define $L\:[0,1] \to \R$ and $\bL \: [0,1] \to \bL^s(\Omega)$ by
%    \begin{equation*}
%      L(t) = \ap{\bL(t),\bvarphi} = \ap{\bLambda_{0,1}(\bv+t\bw),\bvarphi} \quad \text{for all $t\in[0,1]$}.
%    \end{equation*}
%    Let $t\in[0,1]$ and write $\bu = \bv + \hat\bu$. Then,
%    \begin{align*}
%      \abs{\bL(t)} &= \abs{\bLambda_{0,1}(\bv+t\bw)} = \abs{\phi_1(\abs{\bu + t\bw}^2)(\bu+t\bw)}\\
%      &\leq C \abs{\bu + t\bw}^{r-1} + (\lambda_1 + C)\abs{\bu + t\bw}\\
%      &\leq 2^{2-r}C (\abs{\bu}^{r-1} + t^{r-1} \abs{\bw}^{r-1}) + (\lambda_1 + C)(\abs{\bu} + t\abs{\bw})\\
%      &\leq 2^{2-r}C (\abs{\bu}^{r-1} + \abs{\bw}^{r-1}) + (\lambda_1 + C)(\abs{\bu} + \abs{\bw}).
%    \end{align*}
%    The map $[0,1] \ni t \mapsto \abs{\bL(t)}$ is therefore uniformly bounded by a function belonging $L^s(\Omega)$. By Lebesgue's dominated convergence theorem and the continuity of $\phi_1$, we thus get that $\bL$ is continuous and so $L$ is continuous. In other words, $\bLambda_{0,1}$ is hemicontinuous.

%    \medskip
%    \noindent \ul{Monotonicity.} Let $\bv,\bw\in V$. Writing $\bar \bv = \bv + \hat\bu$ and $\bar\bw = \bw +\hat\bu$, we have
%    \begin{align*}
%      \ap{\bLambda_{0,1}(\bv) - \bLambda_{0,1}(\bw),\bv-\bw} &= \int_\Omega ( \phi_1(\abs{\bar \bv}^2) \bar\bv - \phi_1(\abs{\bar \bw}^2) \bar\bw ) \cdot (\bar \bv - \bar \bw)\\
%      &= \int_\Omega \phi_1(\abs{\bar \bv}^2) (\bar\bv - \bar\bw) \cdot (\bar \bv - \bar \bw) + \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot (\bar \bv - \bar \bw)\\
%      &= \int_\Omega \phi_1(\abs{\bar \bv}^2) \abs{\bar\bv - \bar\bw}^2\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot (\bar \bv - \bar \bw)\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot \bar \bv\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) (\abs{\bar\bv}^2 - \abs{\bar \bw}^2)\\
%      &\quad - \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \abs{\bar\bv}^2\\
%      &> \int_\Omega \phi_1(\abs{\bar \bv}^2) \abs{\bar\bv - \bar\bw}^2\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot (\bar \bv - \bar \bw)\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot \bar \bv\\
%      &\quad - \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \abs{\bar\bv}^2\\
%      &= \int_\Omega \phi_1(\abs{\bar \bv}^2) \abs{\bar\bv - \bar\bw}^2\\
%      &\quad - \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \bar\bw \cdot (\bar \bw - \bar \bv)\\
%      &\quad + \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) (\bar\bw-\bar\bv) \cdot \bar \bv\\
%      &= \int_\Omega \phi_1(\abs{\bar \bv}^2) \abs{\bar\bv - \bar\bw}^2\\
%      &\quad - \frac12 \int_\Omega(\phi_1(\abs{\bar \bv}^2) - \phi_1(\abs{\bar \bw}^2)) \abs{\bar \bw - \bar \bv}^2\\
%      &= \frac12 \int_\Omega ( \phi_1(\abs{\bar \bv}^2) + \phi_1(\abs{\bar \bv}^2) ) \abs{\bar\bv - \bar\bw}^2 \geq 0,
%    \end{align*}
%    so that, overall,
%    \begin{equation*}
%      \ap{\bLambda_{0,1}(\bv) - \bLambda_{0,1}(\bw),\bv-\bw} > 0.
%    \end{equation*}
%    Hence $\bLambda_{0,1}$ is strictly monotone. The strict monotonicity stems from the fact that $\phi_1$ is assumed to be strictly increasing.
%  \end{proof}

% \begin{lem}
%   Suppose that $\blambda_1 \preccurlyeq \blambda_2$. The operator $\bLambda_{0,21}$ is maximal.
% \end{lem}

% We thus have shown the existence part of Theorem \ref{thm:wp-1-less-than-2}. The uniqueness part follows from the following lemma:
% \begin{lem}
%   Suppose that $\blambda_1 \preccurlyeq \blambda_2$. The operator $\bLambda_0$ is strongly monotone, that is, there exists $c > 0$ such that
%   \begin{equation*}
%     \ap{\bLambda_{\bv} - \bLambda_{\bw},\bv - \bw} \geq c \norm{\bv - \bw}^2 \quad \text{for all $\bv,\bw\in V$ and all $\bLambda_{\bv} \in \bLambda_0(\bv)$ and $\bLambda_{\bw} \in \bLambda_0(\bw)$}.
%   \end{equation*}
% \end{lem}
% The uniqueness part from \ref{thm:wp-1-less-than-2} is thus proved. Indeed, if two different solutions to Problem \eqref{eq:weak-form-V0} existed, then the strong monotonicity of $\bLambda_0$ would be violated. 



% \section{Single-valued approximation}
% \label{sec:single-valued-approx}

% The question is now to check whether $\bF_*$ satisfies the hypotheses of the Browder--Minty theorem: boundedness, coercivity, hemicontinuity and strict monotonicity. Because of the presence of the Heaviside-like function $H$ in the operator $\bLambda$, we cannot hope for the hemicontinuity of $G$ to hold. For this reason, we shall approximate \eqref{eq:weak-reduced} by a continuous problem.

% Let $H^\e\:\R\to\R$ be a smooth approximation of $H$ converging pointwise to $H$ as the parameter $\e>0$ tends to $0$ and such that $H^\e(1) = h$ (cf. \eqref{eq:heaviside}) for all $\e>0$. For example, if $h=\tfrac12$ then $H^\e$ can be chosen to be the cumulative distribution function of the normal distribution with mean~$1$ and variance $1/\e$. Using from now on upperscripts $\e$ to indicate operators related to the smooth problem, we can write the approximated weak problem, corresponding to \eqref{eq:weak-reduced}: find $\bu^\e\in V^0$ such that
% \begin{equation}
%   \label{eq:weak-reduced-epsilon}
%   \ap{\bF_*^\e(\bu^\e),\bvarphi}_{s,r} = \ap{\bff,\bvarphi}_{s,r} \quad \text{for all $\bvarphi \in V^0$}.
% \end{equation}

% We have the following result:
% \begin{thm}[well-posedness of smooth problem]
%   \label{thm:well-posed-epsilon}
%   Let $\e>0$. There exists a unique $\bu^\e \in V^0$ such that \eqref{eq:weak-reduced-epsilon} holds.
% \end{thm}
% The proof of Theorem \ref{thm:well-posed-epsilon} follows directly from the four lemmas below and the Browder--Minty theorem applied to $\F_*^\e$.

% \begin{lem}[boundedness]
%   Let $\e>0$ and write $S_0$ the unit sphere in $V^0$. The operator $F_*^\e$ is bounded, that is,
%   \begin{equation*}
%     \sup_{\bu \in S_0} \norm{F_*^\e(\bu)}_{L^s(\Omega)} + \norm{F_*^\e(\bnull)}_{L^s(\Omega)} < \infty.
%   \end{equation*}
% \end{lem}

% \begin{lem}[coercivity]
%   Let $\e>0$. The operator $F_*^\e$ is coercive, that is,
%   \begin{equation*}
%     \frac{\ap{F_*^\e(\bu),\bu}_{s,r}}{\norm{\bu}_{L^{r}(\Omega)}} \to \infty \quad \text{as $\norm{\bu}_{L^{r}(\Omega)} \to \infty$}.
%   \end{equation*}
% \end{lem}

% \begin{lem}[hemicontinuity]
%   Let $\e>0$. The operator $F_*^\e$ is hemicontinuous, i.e., the map
%   \begin{equation*}
%     t \mapsto F_*^\e(\bu + t\bv)
%   \end{equation*}
%   is continuous at all $t\in[0,1]$ for all $\bu,\bv \in V^0$.
% \end{lem}

% \begin{lem}[strict monotonicity]
%   Let $\e>0$. The operator $F_*^\e$ is strongly monotone, that is, there exists $C>0$ such that
%   \begin{equation*}
%     \ap{F_*^\e(\bu) - F_*^\e(\bv),\bu - \bv}_{s,r} \geq C\norm{\bu - \bv}_{L^{r}(\Omega)}^2 \quad \text{for all $\bu,\bv\in V^0$}.
%   \end{equation*}
%   In particular, it is strictly monotone.
% \end{lem}


% We shall now show that if $(\bu^\e)_\e \subset V^0$ is a sequence of solutions to \eqref{eq:weak-reduced-epsilon}, then there exists a subsequence of $(\bu_\e)_\e$, still denoted by $(\bu_\e)_\e$, converging to some $\bu\in V^0$ which is solution to \eqref{eq:weak-reduced}.

% \subsection{Browder's theorem}
% \label{sec:browder-thm}

% To show existence of our nonlinear problem we will use the following multivalued extension of the Browder--Minty theorem, due to Browder \comment{referenza: Nonlinear Maximal Monotone Operators in Banach Space} and which we shall therefore refer to as Browder's theorem:
% \begin{thm}[Browder]
%   Let $X$ be a real, separable, reflexive Banach space and let $X^*$ be its dual. Let $T_1$ be a single-valued operator from $X$ to $X^*$ which is bounded, coercive, hemicontinuous and monotone. Let furthermore $T_2$ be a multivalued operator from $X$ to $2^{X^*}$ with $0\in \dom T_2$ which is maximal monotone. Then, the operator $T := T_1 + T_2$ is surjective, i.e.,
%   \begin{equation}
%     \forall\, y\in X^*,\, \exists\, x\in X,\; T(x) = y.
%   \end{equation}
% \end{thm}
% We need to identify the space $X$ and the operator $T$ (and thus $T_1$ and $T_2$) in our setting. To this end, let us introduce the notation $V^0$ for the subset of $L^{r}(\Omega)$ of elements with zero divergence, that is, $\bu\in V^0$ if and only if $\bu \in L^{r}(\Omega)$ and $\ap{\bgrad \psi,\bu}_{s,r} = 0$ for all $\psi\in W^{1,s}(\Omega)$. We show the two lemmas below:
% \begin{lem}
%   \label{lem:bdry-V0}
%   There exists a unique $\bu_*\in L^r(\Omega) \setminus V^0$ such that
%   \begin{equation*}
%     \ap{\bgrad \psi,\bu_*}_{s,r} = -\ap{q,\psi}_{s,r} + \int_{\p\Omega} u_0\psi \quad \text{for all $\psi\in W^{1,s}(\Omega)$}.
%   \end{equation*}
% \end{lem}
% \begin{proof}
%   \comment{da scrivere, seguire la proposizione 3.1 in AFM.}
% \end{proof}
% \begin{lem}
%   The weak formulation \eqref{eq:weak-form-main} is equivalent to the following problem: find $\bu\in V^0$ such that there exists $\phi_* \in \bF(\bu+\bu_*)$ satisfying
%   \begin{equation*}
%     \ap{\phi_*,\bvarphi}_{s,r} = \ap{\bff,\bvarphi}_{s,r} \quad \text{for all $\bvarphi \in V^0$},
%   \end{equation*}
%   where $\bu_*$ is given by Lemma \ref{lem:bdry-V0}.
% \end{lem}
% \begin{proof}
%   \comment{da scrivere, seguire la proposizione 3.2 in AFM.}
% \end{proof}
% Hence the space $X$ and the operator $T$ in Browder's theorem identify in our case with $V^0$ and $\bF_* \: V^0 \to (V^0)^* \sim L^s(\Omega)$, respectively, where
% \begin{equation*}
%   \bF_*(\bu) = \bF(\bu + \bu_*) = \bLambda(\bu + \bu_*)\,(\bu + \bu_*) \quad \text{for all $\bu \in L^{r}(\Omega)$},
% \end{equation*} 
% where again $\bu_*$ is as in Lemma \ref{lem:bdry-V0}. Our problem in weak formulation finally reduces to finding $\bu\in V^0$ such that there exists $\phi_* \in \bF_*(\bu)$ with
% \begin{equation}
%   \label{eq:weak-reduced}
%   \ap{\phi_*,\bvarphi}_{s,r} = \ap{\bff,\bvarphi}_{s,r} \quad \text{for all $\bvarphi \in V^0$}.
% \end{equation}
% We note from \eqref{eq:multiv-heaviside-law} that $\bF_*$ can be written as the sum of a single-valued operator, namely 
% \begin{equation*}
%   \bF_*^1(\bu) := \bF_1(\bu + \bu_*),
% \end{equation*}
% and a multivalued operator, namely 
% \begin{equation*}
%   \bF_*^2(\bu) := \bbH(\abs{\bu + \bu_*}^2) (\bF_2(\bu + \bu_*) - \bF_1(\bu + \bu_*)).
% \end{equation*}
% In Browder's theorem we thus identify $T_1$ and $T_2$ with $\bF_*^1$ and $\bF_*^2$, respectively.

% Since obviously $\bnull \in \dom \bF_*^2$, in order to use Browder's theorem we are left with showing that $\bF_*^1$ is bounded, coercive, hemicontinuous and monotone, and that $\bF_*^2$ is maximal monotone, which we do in the following lemmas. 
% \begin{lem}[boundedness]
%   Write $S^0$ the unit sphere in $V^0$. The operator $\bF_*^1$ is bounded, that is,
%   \begin{equation*}
%     \sup_{\bu \in S_0} \norm{\bF_*^1(\bu)}_{L^s(\Omega)} + \norm{\bF_*^1(\bnull)}_{L^s(\Omega)} < \infty.
%   \end{equation*}
% \end{lem}

% \begin{lem}[coercivity]
%   The operator $\bF_*^1$ is coercive, that is,
%   \begin{equation*}
%     \frac{\ap{\bF_*^1(\bu),\bu}_{s,r}}{\norm{\bu}_{L^{r}(\Omega)}} \to \infty \quad \text{as $\norm{\bu}_{L^{r}(\Omega)} \to \infty$}.
%   \end{equation*}
% \end{lem}

% \begin{lem}[hemicontinuity]
%   The operator $\bF_*^1$ is hemicontinuous, i.e., the map
%   \begin{equation*}
%     t \mapsto \bF_*^1(\bu + t\bv)
%   \end{equation*}
%   is continuous at all $t\in[0,1]$ for all $\bu,\bv \in V^0$.
% \end{lem}

% \begin{lem}[monotonicity]
%   The operator $\bF_*^1$ is strongly monotone, that is, there exists $C>0$ such that
%   \begin{equation*}
%     \ap{\bF_*^1(\bu) - \bF_*^1(\bv),\bu - \bv}_{s,r} \geq C\norm{\bu - \bv}_{L^{r}(\Omega)}^2 \quad \text{for all $\bu,\bv\in V^0$}.
%   \end{equation*}
%   In particular, it is monotone.
% \end{lem}

% \begin{lem}[maximal monotonicity]
%   The operator $\bF_*^2$ is maximal monotone, that is, it is monotone and the operator $\bs{I} + \alpha \bF_*^2$ is surjective for all $\alpha>0$.
% \end{lem}


% which means that we would need to choose an additional law between the velocity field and the pressure field holding in $\Gamma(\bu)$. To avoid this, we impose that
% \begin{equation}\label{eq:gamma-cond}
%   \text{$\Gamma(\bu)$ is $(d-1)$-dimensional},
% \end{equation}
% which in particular implies that $\Gamma(\bu) = \overline\Omega_1(\bu) \cap \overline\Omega_2(\bu)$. We decompose the velocity field $\bu$ as
v% \begin{equation}\label{eq:u-decomp}
% \bu = \bu_1 + \bu_2,
% \end{equation}
% where, for $i\in\{1,2\}$, we define
% \begin{equation}
%   \bu_i = \bu \chi_{\overline \Omega_i(\bu)\setminus\Gamma(\bu)} + \tfrac12 \bu \chi_{\Gamma(\bu)},
% \end{equation}
% where $\chi_A$ stands for the characteristic function of any set $A$. Note that $\bu_1 = \bu_2$ on $\Gamma(\bu)$. We choose the coupled law $\bF$ as
% \begin{equation}\label{eq:F-coupled}
%   \bF = \bF_1\chi_{\Omega_1(\bu)} + \bF_2\chi_{\Omega_2(\bu)},
% \end{equation}
% which gives, for $i\in\{1,2\}$,
% \begin{equation}
%   \bF(\bu) = \bF_1(\bu_1 + \bu_2)\chi_{\Omega_1(\bu)} + \bF_2(\bu_1 + \bu_2)\chi_{\Omega_2(\bu)} = \bF_i(\bu_i) \quad \text{on $\Omega_i(\bu)$},
% \end{equation}
% and thus, Problem \eqref{eq:div-q}--\eqref{eq:no-flux-cond} becomes, if we ignore for now the interface $\Gamma(\bu)$,
% \begin{equation}\label{eq:main}
%   \begin{cases}
%     \dive \bu_i = q & \text{on $\Omega_i(\bu)$},\\
%     \bF_i(\bu_i) = - \bgrad p + \rho \bf & \text{on $\Omega_i(\bu)$},\\
%     \bu_i \cdot \bn = 0 & \text{on $\p\Omega_i(\bu) \cap \Omega$}.
%   \end{cases}
% \end{equation}
% To close the problem \eqref{eq:main} we now need to get interface conditions, in addition to \eqref{eq:gamma-cond}. Analogously to \eqref{eq:u-decomp}, we decompose the pressure as $p = p_1 + p_2$. The definitions of $\bu_1$, $\bu_2$, $p_1$ and $p_2$ suggest that we should impose $\bu_1=\bu_2$ and $p_1=p_2$ on $\Gamma(\bu)$. We shall relax these conditions slightly on the velocity fields $\bu_1$ and $\bu_2$ by only imposing normal and tangent conditions: 
% \begin{equation}\label{eq:interface-cond}
%   \begin{cases}
%     \bu_1 \cdot \bnu = \bu_2 \cdot \bnu,\\
%     \bcurl \bu_1 \times \bnu = \bcurl \bu_2 \times \bnu,\\
%     p_1 = p_2,
%   \end{cases}
%   \quad \text{on $\Gamma(\bu)$},
% \end{equation}
% where $\bnu$ is the outward normal unit vector of $\p\Omega_1$. \comment{[Se ho capito bene, Beavers-Joseph danno condizioni nel caso di un'interfaccia Darcy-Stokes (visto che fanno intevenire il tensore delle tensioni). Nel caso di un'interfaccia generale, per esempio tra Darcy e Darcy-Forchheimer, le condizioni sul curl sopra forse sono più adeguate?]} Our problem of interest in this paper is thus given by \eqref{eq:main}-\eqref{eq:interface-cond} together with the condition \eqref{eq:gamma-cond}.

% \section{The case of two Darcy laws}

% By linearity in this case of the law \eqref{eq:relation-u-p} in the velocity field $\bu$ we get that $\bF$ in \eqref{eq:F-coupled} can written as
% \begin{equation}
%   \bF(\bu) = \mu \bK^{-1}(\bu) \bu,
% \end{equation}
% where the velocity-dependent permeability tensor $\bK(\bu)$ is given by
% \begin{equation}\label{eq:K-darcy-darcy}
%   \bK(\bu) = \bK_1 \chi_{\Omega_1(\bu)} + \bK_2 \chi_{\Omega_2(\bu)}.
% \end{equation}
% We are therefore looking at the following Darcy model:
% \begin{equation}\label{eq:darcy-darcy}
%   \begin{cases} \dive \bu = q,\\ \bK^{-1}(\bu) \bu = -\bgrad p + \rho \bf,\end{cases}
% \end{equation}
% where $\bK(\bu)$ is as in \eqref{eq:K-darcy-darcy}.


% \section{One-dimensional case}
% \label{sec:1d}

% In one dimension, the domain $\Omega$ reduces to an interval. Without loss of generality, we choose $\Omega = (-1,1)$. If we impose $\Gamma(u)$ to be $0$-dimensional, we have $\Gamma(u) = \{\gamma_1(u),\gamma_2(u),\dots\}$ for some family $\{\gamma_k(u)\}_k \subset [-1,1]$. Problem \eqref{eq:main} writes
% \begin{equation}\label{eq:main-1d}
%   \begin{cases}
%     u_i' = q,\\
%     F_i(u_i) = -p' + \rho f,\\
%     u(0) = u(1) = 0,
%   \end{cases}
%   \quad \text{on $\Omega_i(u)$}.
% \end{equation}

% Let us suppose that there exists a solution $(u,p)$. Then, given the boundary conditions, we have
% \begin{equation}
%   \begin{cases}
%     u_1(x) = Q(x) & \text{for all $x\in\Omega_1(u)$},\\
%     u_2(x) = Q(x) & \text{for all $x\in\Omega_2(u)$},
%   \end{cases}
% \end{equation}
% where $Q(x) = \int_{-1}^x q(y) \d y$ for $x\in(-1,1)$ is continuous. We therefore get that
% \begin{equation}
%   \begin{gathered}
%     \Omega_1(u) = \{ x \in (-1,1) \st \abs{Q(x)} < \bar u\}, \quad \text{and} \quad \Omega_2(u) = \{ x \in (-1,1) \st \abs{Q(x)} > \bar u\},\\
%     \Gamma(u) = \{ x \in (-1,1) \st \abs{Q(x)} = \bar u\}.
%   \end{gathered}
% \end{equation}
% We notice that to ensure that $\Gamma(u)$ be $0$-dimensional, we need to choose $q$ and $\bar u$ in such a way that $\abs{Q}$ is almost everywhere different from $\bar u$. For example, we cannot have $Q(a) = \bar u$ for some $a\in(-1,1)$ and then $q(x) = 0$ for all $x\in[a,b]$ with some $b\in(a,1)$.

% \begin{ex}
%   Let us give two examples:
%   \begin{enumerate}
%     \item Choose $q \equiv 0$. Then, $Q \equiv 0$ and since $\bar u > 0$ we have $\Gamma(u) = \Omega_2(u) = \emptyset$ and $\Omega_1(u) = \Omega = (-1,1)$.
%     \item Choose the sigmoid function
%     \begin{equation}
%       q(x) = -\frac12 + \frac{1}{1+e^{-x}} \quad \text{for all $x\in(-1,1)$.}
%     \end{equation}
%     Since $q(x) = 0$ only for $x = 0$, we are safe to say that $\Gamma(u)$ is $0$-dimensional. We know that $\max_{(-1,1)} |Q| = \log(1+e)- 1/2 - \log 2 =: q_*>0$ is achieved at $0$ and we know that, as required, $Q(1) = 0$. Therefore,
%     \begin{equation}
%       \begin{cases}
%         \Gamma(u) = \Omega_2(u) = \emptyset,\; \Omega_1(u) = (-1,1) & \text{if $\bar u > q_*$},\\
%         \Gamma(u) = \{0\},\; \Omega_1(u) = (-1,1),\; \Omega_2(u) = \emptyset & \text{if $\bar u = q_*$},\\
%         \Gamma(u) = \{a,b\},\; \Omega_1(u) = (-1,a) \cup (b,1),\; \Omega_2(u) = (a,b) & \text{if $\bar u < q_*$},
%       \end{cases}
%     \end{equation}
%     where $a = \inf Q^{-1}(\bar u)$ and $b = \sup Q^{-1}(\bar u)$.
%   \end{enumerate}
% \end{ex}

% \comment{[Mi sembra che dati i calcoli sopra il caso 1d sia independente dalla scelta di $F$. In dimensione superiore non sarà sicuramente più il caso.]}

% \section{Well-posedness in dimension one}

% We define the (nonlinear) operator $\Lambda \: L^2(\Omega) \to L^2(\Omega)$ by
% \begin{equation}
%   \Lambda(u) = \lambda_1u + (\lambda_2-\lambda_1) H_{\bar u} \circ u\, u \quad \text{for all $u\in L^2(\Omega)$},
% \end{equation}
% where $H_{\bar u}\: \R \to \R_{\geq 0}$ is given for all $a\in \R$ by
% \begin{equation}
%   H_{\bar u}(a) = \begin{cases} 0 & \text{if $\abs{a} < \bar u$},\\ \frac12 & \text{if $\abs{a} = \bar u$},\\ 1 & \text{if $\abs{a} > \bar u$},\end{cases}
% \end{equation}
% and $\lambda_i\:\Omega\to \R_{\geq 0}$ are inverse permeabilities. The weak formulation of our problem can therefore be rewritten as
% \begin{equation}
%   \begin{gathered}
%     \ap{\Lambda(u),v}_{L^2(\Omega)} + \ap{p',v}_{L^2(\Omega)} = \ap{\rho f,v}_{L^2(\Omega)} \quad \text{for all $v \in L^2(\Omega)$},\\
%     \ap{u,\psi'}_{L^2(\Omega)} = - \ap{q,\psi}_{L^2(\Omega)} \quad \text{for all $\psi \in H^1(\Omega)$}.
%   \end{gathered}
% \end{equation}
% We can show that the problem of finding $(u,p) \in L^2(\Omega)\times H^1(\Omega)$ such that the above equation hold is equivalent to finding $u\in V$ such that
% \begin{equation}\label{eq:weak-1d}
%   \ap{G(u),v}_{L^2(\Omega)} := \ap{K(u+v^*),v}_{L^2(\Omega)} = \ap{\rho f,v}_{L^2(\Omega)},
% \end{equation}
% where $v^*$ is the unique element of $L^2(\Omega)$ satisfying
% \begin{equation}
%   \ap{v^*,\psi'}_{L^2(\Omega)} = - \ap{q,\psi}_{L^2(\Omega)} \quad \text{for all $\psi \in H^1(\Omega)$},
% \end{equation}
% and
% \begin{equation}
%   V = \{ v \in L^2(\Omega) \st \forall\, \psi \in H^1(\Omega),\, \ap{v,\psi'}_{L^2(\Omega)} = 0 \}.
% \end{equation}
% Thanks to \eqref{eq:weak-1d}, the existence of a solution to our problem would stem directly from the surjectivity of the operator $G\: L^2(\Omega) \to L^2(\Omega)$ defined by
% \begin{equation}
%   G(u) = \lambda_1(u+v^*) + (\lambda_2-\lambda_1) H_{\bar u} \circ (u+v^*)\, (u+v^*) \quad \text{for all $u\in L^2(\Omega)$}.
% \end{equation}
% The nonlinearity of $G$ (coming from the jump function $H_{\bar u}$) does not allow us to use the Lax--Milgram theorem. Instead, we shall use the Browder--Minty theorem, which generalizes the former to nonlinear operators. We recall it here:
% \begin{thm}[Browder--Minty]
%   A bounded, coercive, hemicontinuous, monotone operator $T$ from a real, separable, refexive Banach space $X$ into its dual $X^*$ is surjective, i.e.,
%   \begin{equation}
%     \forall\, f\in X^*,\, \exists\, u\in X,\; T(u) = f.
%   \end{equation}
% \end{thm}

% The operator $G$ is easily shown to be bounded and coercive. However, it is not hemicontinuous (again because of $H_{\bar u}$). (It is also probably not monotone.) To overcome this, let us approximate our problem by smoothing $H_{\bar u}$, and thus the operators $\Lambda$ and $G$, as follows:
% \begin{equation}
%   H_{\bar u}^\e(a) = \begin{cases} 0 & \text{if $|a| < \bar u - \e$},\\ \sigma^\e(a) & \text{if $-\bar u - \e < a < -\bar u + \e$ or $\bar u - \e < a < \bar u + \e$},\\ 1 & \text{if $|a| > \bar u + \e$}, \end{cases} 
% \end{equation}
% where $\sigma^\e\:\R\to\R_{\geq 0}$ is a smooth function such that $H_{\bar u}^\e$ is smooth and
% \begin{equation}
%   \sigma^\e(\bar u) = \sigma^\e(-\bar u) = \tfrac12, \quad \sigma^\e(-\bar u - \e) = \sigma^\e(\bar u + \e) = 1 \quad \text{and} \quad \sigma^\e(-\bar u + \e) = \sigma^\e(\bar u - \e) = 0.
% \end{equation}
% The resulting operator $G^\e$ should be continuous and monotone.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "interface_master"
%%% End:

    
